AAFLOW: Scalable Patterns for Agentic AI Workflows

Agentic workflows in large language model systems integrate retrieval, reasoning, and memory, but existing frameworks suffer from scalability and reproducibility limitations due to fragmented data orchestration, serialization overhead, and non-deterministic execution. Although these frameworks increase flexibility, they don't have a formal execution model that adheres to the principles of high-performance computing. We introduce AAFLOW, a unified distributed runtime that creates communication-efficient execution plans by modeling agentic workflows as an operator abstraction. Using Apache Arrow and Cylon, AAFLOW creates a zero-copy data plane that allows direct interoperability between preprocessing, embedding, and vector retrieval without the need for serialization overhead. To lower coordination costs, it uses resource-deterministic scheduling and asynchronous batching. While retaining comparable LLM generation throughput, experimental results demonstrate up to 4.64 times pipeline speedup and 2.8 times gains in embedding and upsert phases. Rather than LLM inference acceleration, these advantages result from enhanced data flow, batching, and communication efficiency.

==> tex/DE_AE/hybrid_async_parallel.tex <==

\section{Parallel Processing Models for Ingestion Pipelines}

We consider an ingestion workload consisting of $N$ items (e.g., documents, chunks, or nodes). The system processes items in batches of size $b$ using up to $P$ parallel workers.

\subsection{Base Cost Model}

Let the cost of processing one batch of size $b$ be
\begin{equation}
T_{\text{batch}}(b) = \alpha + \beta b,
\end{equation}
where:
\begin{itemize}
    \item $\alpha$ is the fixed per-batch overhead (e.g., scheduling, serialization, network setup),
    \item $\beta$ is the per-item processing cost,
    \item $b$ is the batch size.
\end{itemize}

The total number of batches is
\begin{equation}
M = \left\lceil \frac{N}{b} \right\rceil.
\end{equation}

\subsection{Sequential Baseline}

Without batching or parallelism, total execution time is
\begin{equation}
T_{\text{seq}} = N(\alpha + \beta).
\end{equation}

With sequential batching only,
\begin{equation}
T_{\text{seq-batch}} = M(\alpha + \beta b)
\approx \frac{N\alpha}{b} + N\beta.
\end{equation}

\subsection{Bulk Synchronous Parallel (BSP)}

In BSP, computation proceeds in $S$ supersteps. Each superstep consists of:
\begin{enumerate}
    \item parallel local computation,
    \item communication,
    \item a global synchronization barrier.
\end{enumerate}

Let for superstep $s$:
\begin{itemize}
    \item $w_s$ be the total computation workload,
    \item $h_s$ be the communication volume,
    \item $g$ be the communication cost per unit data,
    \item $L$ be the barrier synchronization latency.
\end{itemize}

Then the BSP time for superstep $s$ is
\begin{equation}
T_{\text{BSP}}^{(s)} = \frac{w_s}{P} + g h_s + L.
\end{equation}

Summing over all supersteps:
\begin{equation}
T_{\text{BSP}} = \sum_{s=1}^{S} \left( \frac{w_s}{P} + g h_s + L \right).
\end{equation}

For a three-stage ingestion pipeline (load/transform, embed, upsert), a simple BSP model is
\begin{equation}
\begin{split}
T_{\text{BSP-ingest}} =
\left( \frac{W_1}{P} + gH_1 + L \right)
+ \\
\left( \frac{W_2}{P} + gH_2 + L \right)
+ \\
\left( \frac{W_3}{P} + gH_3 + L \right),
\end{split}
\end{equation}
where $W_i$ and $H_i$ denote the computation and communication costs of stage $i$.

Unlike async pipelines, BSP introduces explicit barrier cost:
\begin{equation}
T_{\text{BSP}} = T_{\text{parallel work}} + T_{\text{communication}} + SL.
\end{equation}

\subsection{Ray-Based Parallel Processing}

Ray models execution as distributed tasks and actors. Let:
\begin{itemize}
    \item $\alpha_r$ be per-task scheduling overhead,
    \item $\beta_r$ be per-item compute cost,
    \item $\sigma_r$ be object-store / serialization overhead per batch,
    \item $\delta_r$ be result collection overhead.
\end{itemize}

If $M$ batches are submitted as Ray tasks, total execution time can be approximated by
\begin{equation}
T_{\text{Ray}} \approx
\left\lceil \frac{M}{P} \right\rceil
(\alpha_r + \sigma_r + \beta_r b)
+ \delta_r.
\end{equation}

Substituting $M \approx \frac{N}{b}$:
\begin{equation}
T_{\text{Ray}} \approx
\frac{N}{bP}(\alpha_r + \sigma_r + \beta_r b) + \delta_r.
\end{equation}

Equivalently,
\begin{equation}
T_{\text{Ray}} \approx
\frac{N(\alpha_r + \sigma_r)}{bP}
+ \frac{N\beta_r}{P}
+ \delta_r.
\end{equation}

This highlights Ray's main tradeoff: it provides flexible distributed parallelism, but incurs explicit task scheduling and object-store overhead.

\subsection{Dask-Based Parallel Processing}

Dask models execution as a task graph. Let:
\begin{itemize}
    \item $\alpha_d$ be per-task scheduling overhead,
    \item $\beta_d$ be per-item compute cost,
    \item $\gamma_d$ be graph construction / dependency management overhead,
    \item $\eta_d$ be communication or shuffle overhead.
\end{itemize}

Then for $M$ batched tasks:
\begin{equation}
T_{\text{Dask}} \approx
\left\lceil \frac{M}{P} \right\rceil
(\alpha_d + \beta_d b)
+ \gamma_d + \eta_d.
\end{equation}

Using $M \approx \frac{N}{b}$:
\begin{equation}
T_{\text{Dask}} \approx
\frac{N}{bP}(\alpha_d + \beta_d b)
+ \gamma_d + \eta_d.
\end{equation}

Equivalently,
\begin{equation}
T_{\text{Dask}} \approx
\frac{N\alpha_d}{bP}
+ \frac{N\beta_d}{P}
+ \gamma_d + \eta_d.
\end{equation}

Dask is effective when task graphs capture substantial coarse-grained parallelism, but communication and graph-management costs become significant when pipelines require many small tasks or frequent shuffles.


\subsection{Async Parallel Batching}

With asynchronous execution and up to $P$ concurrent workers, total time becomes
\begin{equation}
T_{\text{async-batch}} \approx \left\lceil \frac{M}{P} \right\rceil (\alpha + \beta b).
\end{equation}

For large $N$, this simplifies to
\begin{equation}
T_{\text{async-batch}} \approx \frac{N}{bP}(\alpha + \beta b)
= \frac{N\alpha}{bP} + \frac{N\beta}{P}.
\end{equation}

Thus, async batching improves performance in two ways:
\begin{equation}
N\alpha \rightarrow \frac{N\alpha}{bP},
\qquad
N\beta \rightarrow \frac{N\beta}{P}.
\end{equation}


\subsection{Comparative Equation View}

The four execution models can be summarized as follows:

\begin{align}
T_{\text{async-batch}}
&\approx \frac{N\alpha}{bP} + \frac{N\beta}{P}, \\[4pt]
T_{\text{BSP}}
&= \sum_{s=1}^{S}\left(\frac{w_s}{P} + gh_s + L\right), \\[4pt]
T_{\text{Ray}}
&\approx \frac{N(\alpha_r+\sigma_r)}{bP} + \frac{N\beta_r}{P} + \delta_r, \\[4pt]
T_{\text{Dask}}
&\approx \frac{N\alpha_d}{bP} + \frac{N\beta_d}{P} + \gamma_d + \eta_d.
\end{align}

These expressions show that all methods benefit from dividing useful work across $P$ workers, but they differ in the extra overhead terms they introduce:
\begin{itemize}
    \item \textbf{Async batching:} minimized per-batch overhead through concurrency and batching.
    \item \textbf{BSP:} explicit barrier cost $L$ at each superstep.
    \item \textbf{Ray:} task scheduling and object-store overhead.
    \item \textbf{Dask:} graph scheduling and shuffle/communication overhead.
\end{itemize}

\subsection{Pipeline-Level Formulation}

For a multi-stage ingestion pipeline with stages $k \in \{1,\dots,K\}$, the stage cost can be written generically as
\begin{equation}
T_k \approx \frac{N\alpha_k}{b_k P_k} + \frac{N\beta_k}{P_k} + \Omega_k,
\end{equation}
where $\Omega_k$ denotes framework-specific overhead.

Examples include:
\begin{align}
\Omega_k^{\text{async}} &= 0 \quad \text{(idealized)},\\
\Omega_k^{\text{BSP}} &= g h_k + L,\\
\Omega_k^{\text{Ray}} &= \sigma_k + \delta_k,\\
\Omega_k^{\text{Dask}} &= \gamma_k + \eta_k.
\end{align}

Thus, total pipeline time under sequential stage execution is
\begin{equation}
T_{\text{pipeline}} = \sum_{k=1}^{K} T_k.
\end{equation}

If stages are overlapped in an asynchronous pipeline, the total time is closer to
\begin{equation}
T_{\text{pipeline-overlap}} \approx \max_k T_k,
\end{equation}
or more precisely,
\begin{equation}
T_{\text{pipeline-overlap}} \approx T_{\text{startup}} + (M-1)\max_k(t_k) + T_{\text{drain}},
\end{equation}
where $t_k$ is the steady-state time per batch for stage $k$.

Async batching, BSP, Ray, and Dask all reduce execution time by parallelizing work, but their efficiency depends on how much extra coordination overhead they introduce. In general:
\begin{equation}
T = T_{\text{useful work}} + T_{\text{coordination}} + T_{\text{communication}}.
\end{equation}

The performance advantage of async batching comes from minimizing coordination overhead, while BSP, Ray, and Dask trade additional synchronization, scheduling, or graph overhead for more structured and scalable execution.


\section{Implementation}

By parallelizing tokenization, chunking, and embedding processes under a consistent Arrow-based memory model, Cylon guarantees reproducible ETL and preprocessing while ensuring semantic consistency across nodes. This eliminates the nondeterminism that is usually present in pipelines for multi-threaded preprocessing. In the meantime, LlamaIndex's agentic layer substitutes a dynamic, context-aware retrieval engine that modifies its search and ranking approach according to the LLM's reasoning state and historical context for the static retrieval behavior of traditional RAG.

Embedding generation and index creation become totally reproducible and resource-optimized by combining Cylon's distributed communication layer. This greatly reduces time-to-context and improves retrieval accuracy. Additionally, near-real-time index updates and online retraining are made possible by the Arrow-backed data transfer, which reduces serialization overhead between components. Together, these design choices enable the suggested framework to provide agentic, adaptive, and effective RAG pipelines that preserve transparency, scalability, and performance consistency—overcoming the basic obstacles that limit existing LLM retrieval systems.


An integrated stack of distributed data systems, deep learning libraries, and orchestration frameworks is needed to put the above-described architecture into practice(Fig. \ref{fig:aaflow}). The use of open-source technologies to implement these components is explained in the ensuing subsections.

\subsection{Data Processing Layer: Distributed ETL, Embedding and Retrieval Infrastructure}
The RAG pipeline's high-performance data processing activities are supported by the Cylon distributed DataFrame engine. It supports partitioned datasets and group communication via UCX, Gloo, or MPI, enabling effective ETL (Extract, Transform, Load) activities over several nodes. By eliminating I/O and serialization inefficiencies, Cylon's interface with Apache Arrow enables zero-copy data movement between data processing and deep learning modules. This approach facilitates distributed embedding generation with fast throughput and little communication overhead when paired with PyTorch's DataLoader.
Depending on deployment limitations, models from the Sentence-Transformers or OpenAI API are used to compute embeddings. After being normalized, these embeddings are kept in a distributed vector database like FAISS or Pinecone \cite{pinecone2023}. FAISS offers indexing structures (FlatIP, HNSW, IVF) that are geared for high recall and cosine similarity. Dual FAISS indices—one for static knowledge and one for long-term memory embeddings—are used to carry out memory retrieval queries. A retrieval agent uses a weighted scoring system to combine and rank the findings.


\subsection{Information Flow in the Memory-Enhanced RAG Pipeline}

A memory-augmented RAG system's operational lifespan can be thought of as a closed feedback loop that includes memory updates, query comprehension, context retrieval, and reasoning. The following steps are involved in the process:
\textbf{Query Embedding and Contextualization} The system uses an embedding model (such as Sentence-BERT) to encode user queries into a vector representation. In order to ascertain whether the query context is similar to past interactions, the agent simultaneously examines the memory layer. The memory module speeds up inference by providing cached results or previous reasoning traces if a similar query already exists.
\textbf{Dual Retrieval Mechanism: } Two complementary routes emerge from the retrieval process: 1) Knowledge Retrieval: Gets the most recent domain knowledge by accessing the static vector store. 2) Memory Retrieval: Searches on memory for contextual or historical information, such as past user preferences or the results of agentic reasoning.
The technology integrates both factual accuracy and experiential learning thanks to the dual-retrieval approach. The cognitive context of the agent is formed by this hybrid retrieval.

\begin{figure}[htpb]
    \begin{center}
        \includesvg[width=0.9\linewidth]{Figure/Advanced_Async_PP2.svg}
        \end{center}
        \caption{Advanced Async with Parallel Pipeline of AAFLOW. With batching to measure execution time. BE = Size of the batch embeddings; BU = Size of the upsert batching. $T_{Total} = Load\ Time + Transform\ Time(t_1 + t_2) + Index\ Time$}
    \label{fig:async_pp}
\end{figure}

\textbf{Context Synthesis and Reasoning} A composite context window is created by combining the retrieved documents with context from memory. The Reasoning Agent analyzes the combined data via symbolic reasoning, dynamic planning, or chain-of-thought prompting. For traceability, intermediate results like task graphs, extracted entities, or rating scores are recorded in STM.

\textbf{State Updating and Persistence} The agent writes the results back to memory after the task is finished: 1) memory logs instantaneous results for future use. 2) Structured session summaries and compressed embeddings are sent to the vector store. 3) The high-level representation of the reasoning trace is stored in episodic memory.
Continuous adaptation is made possible by this feedback mechanism. The system uses this memory to recreate pertinent states and repurpose learnt patterns in response to subsequent queries.

\textbf{Feedback for Reinforcement and Optimization}
Another important factor in model improvement is memory. For the purpose of retraining or reinforcing, feedback from both successful and unsuccessful responses is encoded and retained. By dynamically modifying similarity thresholds, embedding models, or prompt templates, the agent can assess the efficacy of previous retrieval techniques.


\subsection{AAFLOW's Hybrid Asynchronous Parallel Pipeline}

The hybrid asynchronous parallel pipeline consists of the LlamaIndex parallel ingestion pipeline with adaptive allocation of hardware resources based on availability. It uses bulk embedding generation with parallel batching of upserting operations to the vector store that reduces the number of IO operations and improves performance. There are multiple steps in the pipeline (Fig. \ref{fig:async_pp}):

\textbf{Corpus and Data Generation} setup ensures that all configurations ingest the same number of nodes with the same approximate text size, so timing comparisons are fair. Every run creates a temporary data directory and uses the same synthetic corpus. It targets a total of \texttt{N = ---nodes} logical nodes (chunks), such as 20,000 nodes. These nodes are dispersed over \texttt{---files} text files, such as 200 files. Within each file, a set delimiter separates each logical node, which is a block of random ASCII text of length \texttt{---node-chars} characters (default 800). A custom splitter then uses this delimiter to ensure that the pipeline generates precisely \texttt{N TextNodes}.

\textbf{LlamaIndex Pipeline} is the ingestion front-end, which consists of multiple layers. \textbf{(1) Loading layer} reads the generated text files. \texttt{SimpleDirectoryReader.load\_data()} is used for synchronous loads. \texttt{.load\_data(num\_workers=K)} is used for reader-parallel loads. \textbf{(2) Transform layer} is a single custom splitter transform that uses \texttt{DelimiterNodeSplitter} which inherits from TransformComponent. It splits each document’s raw text by the special delimiter and emits one \texttt{TextNode} per chunk, carrying metadata (\texttt{doc\_index}, \texttt{chunk\_index}, etc.). This splitter is plugged into an IngestionPipeline as:
\texttt{ pipeline = IngestionPipeline(...)} and is executed either:
synchronously via \texttt{pipeline.run(..., num\_workers=...)}, asynchronously via await \texttt{pipeline.arun(..., num\_workers=...)}

\textbf{Embedding Model} part is a bit tricky for a large-scale experiments. To avoid external API variability, the experiments use a FakeEmbedder that simulates a remote embedding service. We set the latency model to \texttt{latency(batch) = request\_overhead\_ms + per\_item\_ms × batch\_size} and use dimension: \texttt{---dim} (default 768). The embedder creates a SHA-256 hash of each supplied text. Deterministically transforms bytes into a dim-length float32 vector in [-1, 1]. In situations when batch size and parallelism are important, this provides repeatable embeddings with a realistic cost profile. Embeddings are created either Sequentially (num\_workers = 1, batch\_size = 1) or with async concurrency (bounded by \texttt{asyncio.Semaphore(num\_workers)}). It can be configured with or without batching (batch\_size configurable).

\textbf{FAISS Vector Store} is an important part of the whole pipeline. ChromaDB is also an alternative. But all experiments use FAISS as the vector index. The base index type is IndexFlatL2 or IndexFlatIP, depending on \texttt{---metric} (l2 or ip). IndexFlatIP is shown to be slightly faster than IndexFlatL2\cite{pinecone_vector_indexes}. Global OpenMP parallelism is configured via \texttt{faiss.omp\_set\_num\_threads(...)}. There are two FAISS backends. \textbf{(1) FaissFlatStore}, a single flat index \texttt{(IndexFlat*)}. Inserts are done via \texttt{index.add()} on batched arrays (\texttt{add\_batch} wrapper). \textbf{(2) FaissShardedStore}, uses multiple shard indexes (IndexFlat*) built in parallel. Combined into an IndexShards index to model BSP-style bulk parallel build. We measure the time to add all embeddings into these indexes under different parallelization patterns.

For each configuration, we record, \texttt{Load time:} directory reader call (sync or parallel), \texttt{Transform time:} run or arun (sync, multiprocessing, or async), \texttt{Embed time:} time spent in the embedding stage, \texttt{FAISS add time:} time spent inserting vectors into the FAISS index, \texttt{Total time:} end-to-end wall-clock.

\section{Performance Evaluation} 


We put up weak and strong scalability utilizing the \texttt{bii-gpu} queue with 37 cores per node and 4 A100s GPUs using UVA Rivanna HPC~\cite{rivanna_2023}. The goal is to assess AAFLOW's effectiveness when doing multitask LLM inferences and compare it to other agentic frameworks, like Langchain\cite{langchain2023}, LangGraph \cite{langgraph2024}, and CreaAI. Two metrics will be measured: DRC overheads and throughputs, as well as total and average execution time. The Total Execution Time shows how much time AAFLOW spent using the computational resources to carry out the LLM inference and data pretreatment activities. The overheads show how long it takes DRC to (i) deserialize the task object and (ii) build the \texttt{Communicator} with N rankings and send it to the tasks. The average time required by all N levels is represented by the average execution time. N ranks are required for each agentic job, with a maximum of 10,000 inferences per rank. 

A series of tests was carried out on heterogeneous high-performance computing (HPC) and multi-GPU clusters to evaluate the resilience and performance of the suggested Agentic RAG Framework. The studies focused on three aspects: (1) distributed preprocessing throughput, (2) retrieval latency and accuracy, and (3) scalability and repeatability under dynamic workloads. They mainly evaluated the framework against conventional RAG and standard LLM inference pipelines. Using Cylon for distributed ETL and embedding generation and LlamaIndex for resource orchestration, the system was implemented on HPC systems.
\begin{table}[t]
\centering
\caption{Quantitative results (64 test runs) on 2×A100 80GB GPUs, 8-core node.}
\label{tab:overall_results}
\scriptsize
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{\textbf{Baseline}} 
& \multicolumn{2}{c}{\textbf{AAFLOW}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Framework} & Lat (s) & Thr (req/s) & Lat (s) & Thr (req/s) \\
\midrule
LangGraph  & 1.707 & 0.586 & 1.690 & 0.587 \\
LangChain  & 1.708 & 0.586 & 1.698 & 0.588 \\
AutoGen    & 1.575 & 0.635 & 1.412 & 0.672 \\
CrewAI     & 1.574 & 0.635 & 1.487 & 0.691 \\
LlamaIndex & 1.196 & 0.836 & 1.098 & 0.861 \\
\bottomrule
\end{tabular}
\end{table}


\begin{comment}
\subsection{Distributed Preprocessing and ETL Throughput} 

Data preparation and embedding creation, which are usually carried either sequentially or with coarse-grained parallelism, are two of the main bottlenecks in traditional RAG systems. The suggested system achieves near-linear scaling in ETL activities including document chunking, tokenization, and vector embedding by utilizing Cylon's distributed dataframe and Arrow-based memory architecture. Preprocessing throughput increased by about 6\% with 10\% less latencies on an 8-node cluster (Fig.- \ref{fig:cylon_latency_throughput}) compared to the baseline RAG pipeline implemented with Python multiprocessing. Using Cylon operators, we have introduced document load, cleaning, and chunk creation to the RAG pipeline.  Cylon's capacity to reduce serialization overhead and preserve memory locality during transformation and shuffle operations is the source of this gain.






\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=1 by 2,
    vertical sep=1.0cm
  },
  ybar,
  width=\columnwidth,
  height=0.55\columnwidth,
  bar width=5pt,
  ymode=log,
  symbolic x coords={Docs,Chunks},
  xtick=data,
  xticklabel style={font=\footnotesize},
  tick label style={font=\footnotesize},
  ymajorgrids=true,
  legend style={
    at={(0.5,1.2)},
    anchor=south,
    legend columns=2,
    font=\footnotesize
  },
]

% ---------------- Latency Panel ----------------
\nextgroupplot[
  title={Latency},
  title style={font=\footnotesize},
  ylabel={Seconds (log scale)},
  ylabel style={font=\footnotesize},
]
\addplot[fill=red] coordinates {
  (Docs,   2.07115e-05)
  (Chunks, 6.53323e-07)
};
\addplot[fill=green] coordinates {
  (Docs,   1.69046e-05)
  (Chunks, 5.48730e-07)
};
\legend{Agentic DRC, Async Parallel}

% ---------------- Throughput Panel ----------------
\nextgroupplot[
  title={Throughput},
  title style={font=\footnotesize},
  ylabel={Tokens/s (log scale)},
  ylabel style={font=\footnotesize},
]
\addplot[fill=red] coordinates {
  (Docs,   4.82822e+04)
  (Chunks, 1.43064e+06)
};
\addplot[fill=green] coordinates {
  (Docs,   5.28275e+04)
  (Chunks, 1.60231e+06)
};

\end{groupplot}
\end{tikzpicture}

\caption{Latency and throughput comparison for Docs and Chunks workloads with and without Cylon acceleration. Log-scale emphasizes magnitude differences and relative performance improvement.}
\label{fig:cylon_latency_throughput}
\end{figure}

Furthermore, concurrent execution of embedding generation and index construction across worker nodes was made possible by RADICAL-Pilot's dynamic task scheduling. Through pilot-level telemetry, this will decrease idle time and increase resource use efficiency. RADICALPilot.TaskDescription's structured description of ETL tasks will enable exact control over GPU and CPU allocations, guaranteeing deterministic and repeatable execution over several runs.

\end{comment}

\subsection{Token Generation Benchmarking}

The AAFLOW workload's token generation findings demonstrate how multi-step reasoning, retrieval, and orchestration significantly alter the performance profile of big language models. A total of 512,013 tokens were generated over 23,459 seconds over 400 agentic generations, resulting in an average delay of 58.6 seconds per generation and an effective throughput of roughly 21.8 tokens per second (table-\ref{tab:agentic_async_raw}). This token-per-second rate seems low when compared to benchmarks for raw decoding, which can surpass 80 to 120 tokens per second on contemporary GPUs; nevertheless, the difference is due to the structural overhead that comes with agentic pipelines.

AAFLOW imposes a reasoning-driven workflow consisting of contextual retrieval, multi-phase planning, validation, and reflective refinement, in contrast to standard LLM inference, where a model streams tokens constantly following a single prefill step. These actions cause additional prefill stages, rebuild or enlarge context windows, and generate computational pauses in between token bursts. Consequently, a considerable amount of the overall generation time is not used for pure decoding. Additionally, the cost of large-context attention, KV-cache maintenance, and post-hoc agent activities like summarization, formatting, or tool invocation is increased by the average output length of about 1,280 tokens per generation.
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    width=\columnwidth,
    height=0.55\columnwidth,
    bar width=6pt,
    symbolic x coords={Tokens/sec,Avg Latency (s),Total Time (s)},
    xtick=data,
    xticklabel style={rotate=20, anchor=east, font=\footnotesize},
    ylabel={Relative value (Async Parallel = 1.0)},
    ylabel style={font=\footnotesize},
    ymin=0,
    enlarge x limits=0.15,
    legend style={
        at={(0.5,1.03)},
        anchor=south,
        legend columns=2,
        font=\footnotesize
    },
    ymajorgrids=true,
    tick label style={font=\footnotesize}
]

% Agentic DRC
\addplot[fill=green] coordinates {
    (Tokens/sec,1.17997)
    (Avg Latency (s),0.84746)
    (Total Time (s),0.84746)
};

% Async Parallel baseline
\addplot[fill=red] coordinates {
    (Tokens/sec,1.0)
    (Avg Latency (s),1.0)
    (Total Time (s),1.0)
};

\legend{AAFLOW, Async Parallel}

\end{axis}

% Reference line at 1.0
\draw[dashed,gray] (rel axis cs:0,1) -- (rel axis cs:1,1);

\end{tikzpicture}
\caption{Comparison of AAFLOW and Async Parallel execution modes, normalized such that Async Parallel = 1.0 for all metrics from Table~\ref{tab:agentic_async_raw}. AAFLOW achieves higher throughput and lower latency and total runtime.}
\label{fig:agentic_vs_async}
\end{figure}




Therefore, the effective throughput of 21.8 tokens per second should be seen as a measure of cognitive labor done per agentic graph rather than as poor raw model performance. Actually, this rate is in line with expectations for reflective, multi-step, tool-aware agent systems, where the objective is to reason, retrieve, verify, and plan in addition to producing text quickly. In this way, AAFLOW represents a change from language models as "typewriters" to language models as adaptive cognitive engines by trading continuous decode speed for organized decision-making.

\begin{table}[t]
\centering
\caption{Original performance metrics for AAFLOW and Async Parallel. Time in seconds; throughput in tokens/s.}
\label{tab:agentic_async_raw}
\scriptsize
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{lcc}
\toprule
\textbf{Metric} & \textbf{AAFLOW} & \textbf{Async Parallel} \\
\midrule
Total tokens & 512{,}013 & 512{,}012 \\
Total time & 23{,}459.54 & 27{,}682.25 \\
Generations & 400 & 400 \\
Avg latency / gen & 58.65 & 69.21 \\
Tokens/s & 21.82 & 18.50 \\
\bottomrule
\end{tabular}
\end{table}
\begin{comment}



\subsection{Retrieval Latency and Context Adaptation}

In retrieval experiments using LamaIndex’s agentic retriever, which dynamically selects data sources based on LLM reasoning feedback, the proposed architecture demonstrated substantial gains in both retrieval accuracy and inference latency. Compared to a static FAISS-based retriever, the agentic RAG framework achieved a 23\% reduction in mean retrieval latency and a 17\% improvement in top-k retrieval precision across benchmark datasets (e.g., PubMedQA and WikiText).

This gain can be attributed to two key design decisions: (1) adaptive retrieval strategies, where the LLM’s chain-of-thought or reasoning trace influences query reformulation and ranking order, and (2) Arrow-backed in-memory communication between Cylon and LamaIndex, eliminating redundant deserialization. The integration with RADICAL-Pilot ensures that high-priority retrieval operations receive dedicated compute resources during multi-agent inference sessions, minimizing queuing delays and improving throughput.  

\subsection{Scalability and Reproducibility}

Scalability tests showed that the framework maintained consistent performance up to 128 concurrent nodes without degradation in throughput or retrieval accuracy \cite{johnson2019faiss}. The multi-node communicator management implemented in RADICAL-Pilot allowed efficient orchestration of concurrent distributed operators (e.g., shuffle, reduce, gather) used during RAG preprocessing and embedding refresh. Importantly, the framework exhibited reproducible embedding consistency across distributed environments—where embedding vector drift between independent runs dropped from 2.7\% (baseline) to 0.4\% (proposed), as measured via cosine distance metrics.

Moreover, reproducibility under dynamic workloads—where resources were scaled elastically—remained intact due to the deterministic nature of task allocation and the use of consistent random seeds across distributed ranks. This property is essential for scientific and industrial RAG pipelines, where traceability and explainability are as critical as performance.

\subsection{End-to-End System Efficiency}

End-to-end evaluations integrating data ingestion, preprocessing, retrieval, and inference demonstrated an overall 2.9× improvement in system-level efficiency compared to standard RAG pipelines. The hybrid orchestration of Cylon + RADICAL-Pilot not only reduced end-to-end latency but also provided fine-grained control over resource binding, resulting in predictable and explainable performance profiles.

Collectively, these results confirm that the proposed Agentic RAG Framework successfully addresses the major inefficiencies of current LLM retrieval architectures—providing a scalable, reproducible, and semantically consistent approach to distributed reasoning and adaptive context management.

\section{Discussion and Future Work} 

The integration of Cylon, LamaIndex, and RADICAL-Pilot within the Agentic RAG Framework demonstrates that distributed data preprocessing, adaptive retrieval, and dynamic orchestration can coexist within a unified architecture for large-scale LLM applications. The empirical findings highlight the significant efficiency gains achievable through deterministic ETL pipelines and context-aware retrieval mechanisms. However, several important challenges remain—particularly in scalability, generalization, and cross-domain adaptability—that open pathways for future investigation.

\subsection{Interpretability and Adaptive Control}

One of the emerging frontiers is the interpretability of agentic retrieval behavior. While the current system employs adaptive retrieval through LamaIndex’s agentic reasoning layer, the decision-making process behind query reformulation and context ranking is often opaque. Future work will explore explainable retrieval controllers that trace decision logic, providing insights into why specific context sources were selected. Integrating reinforcement learning from human feedback (RLHF) or self-corrective retrieval mechanisms could further enhance interpretability while ensuring alignment with user intent and factual consistency.

\subsection{Federated and Cross-Domain Data Orchestration}

The present framework primarily targets HPC-based distributed infrastructures; however, many enterprise and research use cases involve federated or hybrid data environments spread across multiple security domains. Extending Cylon’s distributed ETL layer to operate over federated learning settings—where data remains decentralized but feature spaces must be harmonized—represents a crucial next step. Incorporating privacy-preserving protocols such as differential privacy or secure multiparty computation (SMPC) would enable broader adoption in sensitive data contexts, including healthcare and finance. Moreover, expanding the System Bridge abstraction to support multi-cloud orchestration could allow RADICAL-Pilot to dynamically allocate resources between cloud and HPC nodes while preserving reproducibility guarantees.

\subsection{Integration with Vector Databases and Knowledge Graphs}

Although the current implementation relies on LamaIndex’s in-memory retrieval subsystem, future iterations aim to integrate distributed vector databases such as Milvus, Pinecone, or FAISS-GPU to support petabyte-scale retrieval. Such integration will enable the agentic RAG to operate on knowledge graphs and structured enterprise data, extending its reasoning capability beyond unstructured text. Embedding synchronization between the Cylon ETL layer and external vector databases will also be optimized through Arrow Flight RPC, ensuring zero-copy data interchange and consistent vector space alignment across distributed environments.

\subsection{Real-Time Adaptive Inference and Feedback Loops}

Another critical research trajectory involves enabling real-time feedback loops where the agentic retriever dynamically adjusts its context window and reasoning scope during ongoing inference. Coupling LamaIndex’s agent layer with low-latency telemetry streams from RADICAL-Pilot could allow inference-time adaptation to resource availability or contextual novelty. This would create self-regulating agentic pipelines capable of reasoning under uncertainty, resource constraints, or evolving data distributions—moving toward a new class of autonomous reasoning systems for HPC and AI research.

\subsection{Theoretical Advancements and Benchmarks}

While empirical evaluations confirm the system’s scalability and reproducibility, further theoretical analysis is required to establish optimal bounds for communication complexity, embedding drift, and retrieval convergence under distributed operations. Developing a standardized Agentic RAG Benchmark Suite—covering metrics such as semantic stability, resource elasticity, and retrieval precision under varying loads—will provide a rigorous foundation for comparative evaluation against future architectures. Additionally, leveraging graph-based task scheduling models could improve reasoning efficiency by reducing redundant dependency resolution between distributed tasks.

\subsection{Toward a Unified Agentic-HPC Ecosystem}

Ultimately, the convergence of agentic AI frameworks and HPC middleware offers a promising pathway toward a Unified Agentic-HPC Ecosystem, where distributed AI workflows are treated as dynamic, self-optimizing processes. Future research will explore meta-orchestration, where multiple agentic subsystems—such as retrieval, summarization, and decision agents—operate under a shared control policy managed by RADICAL-Pilot. This paradigm could enable large-scale multi-agent collaboration with adaptive data routing and workload balancing across heterogeneous compute environments.

In summary, the proposed method establishes the foundation for scalable, adaptive, and reproducible RAG systems that bridge HPC and AI research. By integrating deterministic data engineering (Cylon), adaptive retrieval (LamaIndex), and dynamic orchestration (RADICAL-Pilot), the proposed framework not only mitigates the inefficiencies of current LLM pipelines but also opens new directions in distributed reasoning, interpretability, and self-organizing AI infrastructure.
\end{comment}





%\section{Pipeline Benchmarking with Multiple Operations}

\subsection{AAFLOW Hybrid Parallel Ingestion Pipeline Benchmarking}
The controlled synthetic ingestion pipeline used in the tests allows for the isolation and comparison of various parallelization strategies (Configs 1–5) without being influenced by other services or network noise. 
\begin{table*}[t]
\centering
\caption{Benchmark comparison across parallel configurations (5000 chunks, 200 files).}
\label{tab:parallel_benchmarks}
\scriptsize
\setlength{\tabcolsep}{13pt}
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{
    l
    S[table-format=4.0]
    S[table-format=3.3]
    S[table-format=3.3]
    S[table-format=3.3]
    S[table-format=3.3]
    S[table-format=3.3]
    S[table-format=2.2]
    l
}
\toprule
\textbf{Config}
 & \textbf{Chunks}
 & {\textbf{Load}}
 & {\textbf{Trans.}}
 & {\textbf{Embed}}
 & {\textbf{Upsert}}
 & {\textbf{Total}}
 & {\textbf{Speedup}}
 & {$\Delta$ vs Base} \\
 &  & {(s)} & {(s)} & {(s)} & {(s)} & {(s)} & {($\times$)} &  \\
\midrule

LoaderParallel           
 & 5000 & 5.246  & 0.127  & 311.319 & 43.673 & 366.789 & 1.00  & baseline \\

ReaderParallel           
 & 5000 & 32.667 & 0.051  & 311.490 & 45.712 & 389.988 & 0.94  & $-6.3\%$ \\

PipelineParallelSync     
 & 5000 & 0.010  & 26.945 & 311.457 & 46.957 & 385.447 & 0.95  & $-5.1\%$ \\

AsyncParallelOnly        
 & 5000 & 0.010  & 0.898  & 10.093  & 47.489 & 58.545  & 6.27  & $84.0\%$ \\

\textbf{AAFLOW}      
 & 5000 & 0.010  & 0.979  & 0.737   & 5.594  & \textbf{7.376} 
 & \textbf{49.73} & \textbf{98.0\%} \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\scriptsize \textit{AAFLOW vs AsyncParallelOnly total improvement: $87.4\%$ faster.}
\end{table*}
The most notable distinction between AAFLOW and AsyncParallelOnly is that AAFLOW modifies the workload's structure to require significantly less computing in the first place, rather than just running the same pipeline more quickly. The Load, Transform, Embed, and Upsert phases all reflect this disparity in different ways.

\textbf{(1) Load:} AAFLOW does not rely on aggressive prefetching or parallel file I/O to achieve near-zero (\~0.01s) data loading overhead in 3rd column of table-\ref{tab:parallel_benchmarks}. Rather, it issues fewer load operations and eliminates superfluous payloads. Meanwhile, by overlapping I/O with concurrent embedding operations, AsyncParallelOnly removes the majority of the load stall. Data motion is no longer the primary cost driver for either design at this granularity, as evidenced by parity.

\textbf{(2) Transform:} With sub-second performance (0.898s), AsyncParallelOnly still completes the entire set of transformations for every node. The fact that AAFLOW is still in the same order of magnitude (0.979s) suggests that the breakthrough did not happen during transformation (4th Column in table-\ref{tab:parallel_benchmarks}). The key distinction is qualitative rather than quantitative: AsyncParallelOnly modifies everything but conceals latency through concurrency, whereas AAFLOW conditionally transforms only the subsets of nodes needed for reasoning. This suggests a deeper theme: AsyncParallelOnly parallelizes work, while AAFLOW avoids it.

\textbf{(3) Embed:} The gap becomes crucial during the embedding stage. By using concurrency, AsyncParallelOnly reduces embedding from hundreds of seconds to about ten seconds. On top of an already highly optimized asynchronous baseline, AAFLOW achieves more than an order of magnitude increase by collapsing embedding to less than a second (0.737s, 5th column in table-\ref{tab:parallel_benchmarks}). Instead of executing numerous embeddings in simultaneously, the agentic planner minimizes the size and frequency of embeddings, making this feasible. It executes planning, summarization, and retrieval processes that produce significantly fewer tokens and vectors for encoding. AAFLOW effectively reduces token × embedding procedures, although AsyncParallelOnly reduces wall-clock embedding wait.

\textbf{(4) Upsert:} When embedding is removed as the bottleneck, AsyncParallelOnly's enormous upsert tail (47.489s) becomes the dominating residual cost. By inserting far fewer vectors and carrying out less redundant storage work, AAFLOW decreases upsert to 5.594s(6th column in table-\ref{tab:parallel_benchmarks}), which is almost an order of magnitude less. Once more, this is an example of workload reduction as opposed to aggressive scheduling. AAFLOW saves high-value representations created from reasoning in a chosen manner rather than overloading the datastore with parallelized material.

We observed that when the system moves from non-parallel execution to increasingly more structured and intelligent parallelism, the benchmark results in the table-\ref{tab:parallel_benchmarks} %and Fig.-\ref{fig:parallel_3x2_metrics} 
show a significant performance gain. For 5000 chunks, the basic configuration (LoaderParallel) results in a total runtime of 366.8 seconds, with embedding and upsert operations accounting for nearly all of this time. With runtime reductions of 6.3\% and 5.1\%, respectively, ReaderParallel and PipelineParallelSync provide modest gains. Both approaches have a crucial flaw, though: although adding parallelism, they don't significantly lessen the embedding bottleneck. The majority of wall time is still devoted to waiting for compute phases that are either poorly scheduled or serialized. Only when parallelism is asynchronous does meaningful acceleration manifest. By removing important blocking dependencies and reducing embedding time by almost an order of magnitude, AsyncParallelOnly improves wall time to 58.5 seconds and provides a 6.27× speedup over the baseline. While upsert operations continue to be the primary residual cost, pipeline breaking and parallel scheduling are most beneficial for the transformation and embedding phases. The AAFLOW configuration, which yields a total runtime of just 7.38 seconds—a 49.7× speedup over the baseline and an 87.4\% gain over AsyncParallelOnly—is the most significant performance boost. The main difference is that AAFLOW reorganizes the workload to reduce needless computation rather than just parallelizing execution. Upserts are decreased by almost an order of magnitude and embedding time is cut from tens of seconds to less than one second, indicating savings in unnecessary or duplicated work rather than raw parallel throughput.


When combined, these findings demonstrate that while naive parallelism is beneficial, agentic reorganization significantly alters the pipeline's computational cost profile. AAFLOW transforms parallelism from a technique to "do more things at once" into a way to "perform less overall work effectively," producing the biggest advantages, by lowering token and embedding volume, coordinating work, and removing blocking dependencies.


\subsection{Scaling AAFLOW Parallel Ingestion with multiple operators}
AAFLOW is co-designed for model-driven ingestion pipelines, i.e., workloads where the critical path is not pure ETL but rather Load → Transform → Embed → Upsert into a vector or semantic store, as opposed to popular data processing and serving frameworks like  Dataproc/Spark, Ray, Dask, and GPU-centric ingestion pipelines (e.g., Triton Inference–backed ETL and custom CUDA ingestion stacks). Conventional ETL frameworks (Spark/Dataproc) and DAG execution engines (Ray/Dask) maintain bulk-synchronous execution at stage boundaries while concentrating on throughput maximization through task-level scheduling and shuffle parallelism. Similarly, end-to-end queueing semantics and cross-node coordination are absent from TF Data and PyTorch DataLoader pipelines, which optimize single-node batching into model inference. High FLOP/throughput rates for embedding and inference are provided by GPU ingestion pipelines and Triton deployments, but they handle Load, Transform, and Upsert as external issues, leaving users to piece services together using ad hoc queues, backpressure, and retry policies.


\begin{figure*}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style = {
    group size = 3 by 2,
    horizontal sep = 1.6cm,
    vertical sep = 2.2cm
  },
  width=0.32\linewidth,
  height=0.25\linewidth,
  xmode=log,
  log basis x=2,
  xmin=1, xmax=4096,
  xtick={1,2,4,8,16,32,64,128,256,512,1024,2048,4096},
  xticklabels={1,2,4,8,16,32,64,128,256,512,1024,2048,4096},
  xticklabel style={rotate=90, anchor=east},
  grid=both,
  legend cell align={center},
  legend style={
    font=\scriptsize,
    legend columns=5,
    at={(1.8,1.18)},
    anchor=south,
    draw=none,
    column sep=0.35cm
  },
  xlabel={No of Chunks}
]

% ------------------------------------------------------------------
% 1) LOAD
% ------------------------------------------------------------------
\nextgroupplot[
  title={Load},
  ylabel={Time (s)},
  ymode=log
]

\addlegendentry{NoParallel}
\addlegendentry{ReaderParallel}
\addlegendentry{PipelineParallelSync}
\addlegendentry{AsyncParallelOnly}
\addlegendentry{AgenticDRC}

\addplot[red, thick,mark=*] coordinates {
  (1,4.191)(2,4.459)(4,4.31)(8,3.978)
  (16,4.453)(32,4.298)(64,4.521)(128,4.475)
  (256,4.207)(512,4.605)(1024,4.609)(2048,4.443)
  (4096,4.092)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,30.823)(2,30.932)(4,30.661)(8,31.277)
  (16,30.909)(32,31.413)(64,31.452)(128,30.973)
  (256,32.135)(512,32.117)(1024,31.816)(2048,31.45)
  (4096,30.815)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.006)(2,0.006)(4,0.006)(8,0.006)
  (16,0.006)(32,0.006)(64,0.006)(128,0.006)
  (256,0.008)(512,0.008)(1024,0.008)(2048,0.008)
  (4096,0.009)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.006)(2,0.006)(4,0.006)(8,0.006)
  (16,0.006)(32,0.006)(64,0.006)(128,0.006)
  (256,0.006)(512,0.008)(1024,0.008)(2048,0.008)
  (4096,0.009)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.006)(2,0.006)(4,0.006)(8,0.006)
  (16,0.006)(32,0.006)(64,0.006)(128,0.007)
  (256,0.007)(512,0.007)(1024,0.009)(2048,0.008)
  (4096,0.01)
};

% ------------------------------------------------------------------
% 2) TRANSFORM
% ------------------------------------------------------------------
\nextgroupplot[
  title={Transform},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,0.001)(2,0.001)(4,0.001)(8,0.001)
  (16,0.001)(32,0.001)(64,0.001)(128,0.002)
  (256,0.003)(512,0.007)(1024,0.013)(2048,0.022)
  (4096,0.113)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.0)(2,0.0)(4,0.0)(8,0.001)
  (16,0.001)(32,0.001)(64,0.001)(128,0.002)
  (256,0.003)(512,0.005)(1024,0.103)(2048,0.019)
  (4096,0.13)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,25.201)(2,25.043)(4,25.182)(8,24.935)
  (16,24.685)(32,25.628)(64,25.464)(128,25.353)
  (256,25.769)(512,25.367)(1024,25.803)(2048,26.345)
  (4096,26.341)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.247)(2,0.244)(4,0.248)(8,0.257)
  (16,0.248)(32,0.258)(64,0.254)(128,0.281)
  (256,0.283)(512,0.339)(1024,0.392)(2048,0.498)
  (4096,0.678)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.252)(2,0.248)(4,0.247)(8,0.263)
  (16,0.25)(32,0.254)(64,0.265)(128,0.286)
  (256,0.289)(512,0.345)(1024,0.4)(2048,0.614)
  (4096,0.727)
};

% ------------------------------------------------------------------
% 3) EMBED
% ------------------------------------------------------------------
\nextgroupplot[
  title={Embed},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,0.062)(2,0.125)(4,0.249)(8,0.498)
  (16,0.998)(32,1.992)(64,3.984)(128,7.967)
  (256,15.935)(512,31.875)(1024,63.75)(2048,127.59)
  (4096,255.0)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.062)(2,0.125)(4,0.249)(8,0.498)
  (16,0.996)(32,1.992)(64,3.983)(128,7.965)
  (256,15.935)(512,31.876)(1024,63.751)(2048,127.513)
  (4096,255.082)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.062)(2,0.125)(4,0.249)(8,0.498)
  (16,0.996)(32,1.991)(64,3.989)(128,7.966)
  (256,15.934)(512,31.964)(1024,63.752)(2048,127.562)
  (4096,255.063)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.062)(2,0.062)(4,0.063)(8,0.063)
  (16,0.063)(32,0.065)(64,0.129)(128,0.257)
  (256,0.516)(512,1.032)(1024,2.067)(2048,4.139)
  (4096,8.325)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.063)(2,0.063)(4,0.066)(8,0.071)
  (16,0.081)(32,0.101)(64,0.141)(128,0.145)
  (256,0.153)(512,0.17)(1024,0.202)(2048,0.277)
  (4096,0.54)
};

% ------------------------------------------------------------------
% 4) UPSERT
% ------------------------------------------------------------------
\nextgroupplot[
  title={Upsert},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,0.005)(2,0.007)(4,0.01)(8,0.018)
  (16,0.035)(32,0.071)(64,0.152)(128,0.351)
  (256,0.903)(512,2.595)(1024,8.139)(2048,16.688)
  (4096,34.448)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.004)(2,0.006)(4,0.01)(8,0.018)
  (16,0.034)(32,0.073)(64,0.151)(128,0.362)
  (256,0.917)(512,2.687)(1024,8.397)(2048,17.164)
  (4096,35.709)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.003)(2,0.005)(4,0.009)(8,0.017)
  (16,0.033)(32,0.069)(64,0.151)(128,0.366)
  (256,0.955)(512,2.75)(1024,8.618)(2048,17.576)
  (4096,37.311)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.004)(2,0.006)(4,0.011)(8,0.019)
  (16,0.038)(32,0.074)(64,0.167)(128,0.363)
  (256,0.936)(512,2.724)(1024,8.529)(2048,17.573)
  (4096,37.463)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.004)(2,0.005)(4,0.006)(8,0.007)
  (16,0.012)(32,0.021)(64,0.041)(128,0.096)
  (256,0.202)(512,0.439)(1024,0.902)(2048,1.97)
  (4096,4.286)
};

% ------------------------------------------------------------------
% 5) TOTAL
% ------------------------------------------------------------------
\nextgroupplot[
  title={Total},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,7.971)(2,8.143)(4,9.467)(8,8.582)
  (16,9.329)(32,11.36)(64,15.662)(128,17.829)
  (256,25.68)(512,47.276)(1024,81.662)(2048,155.056)
  (4096,298.708)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,30.895)(2,31.068)(4,30.944)(8,31.799)
  (16,31.945)(32,33.486)(64,35.593)(128,39.307)
  (256,48.998)(512,66.695)(1024,104.082)(2048,176.171)
  (4096,321.797)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,25.278)(2,25.183)(4,25.462)(8,25.46)
  (16,25.726)(32,27.699)(64,29.615)(128,33.697)
  (256,42.673)(512,60.105)(1024,98.202)(2048,171.532)
  (4096,318.787)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.34)(2,0.323)(4,0.332)(8,0.349)
  (16,0.36)(32,0.408)(64,0.577)(128,0.913)
  (256,1.748)(512,4.129)(1024,11.037)(2048,22.261)
  (4096,46.528)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.329)(2,0.333)(4,0.339)(8,0.353)
  (16,0.353)(32,0.387)(64,0.459)(128,0.555)
  (256,0.679)(512,0.995)(1024,1.545)(2048,2.906)
  (4096,5.624)
};

% ------------------------------------------------------------------
% 6) SPEEDUP VS BASELINE
% ------------------------------------------------------------------
\nextgroupplot[
  title={Speed vs baseline},
  ylabel={Speedup ($\times$)},
  ymin=0
]

\addplot[red, thick,mark=*] coordinates {
  (1,1)(2,1)(4,1)(8,1)
  (16,1)(32,1)(64,1)(128,1)
  (256,1)(512,1)(1024,1)(2048,1)
  (4096,1)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.2580)(2,0.2621)(4,0.3059)(8,0.2699)
  (16,0.2920)(32,0.3392)(64,0.4400)(128,0.4536)
  (256,0.5241)(512,0.7088)(1024,0.7846)(2048,0.8801)
  (4096,0.9282)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.3153)(2,0.3234)(4,0.3718)(8,0.3371)
  (16,0.3626)(32,0.4101)(64,0.5289)(128,0.5291)
  (256,0.6018)(512,0.7866)(1024,0.8316)(2048,0.9039)
  (4096,0.9370)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,23.4441)(2,25.2105)(4,28.5151)(8,24.5903)
  (16,25.9139)(32,27.8431)(64,27.1438)(128,19.5279)
  (256,14.6911)(512,11.4497)(1024,7.3989)(2048,6.9654)
  (4096,6.4200)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,24.2280)(2,24.4535)(4,27.9263)(8,24.3116)
  (16,26.4278)(32,29.3540)(64,34.1220)(128,32.1243)
  (256,37.8203)(512,47.5136)(1024,52.8557)(2048,53.3572)
  (4096,53.1131)
};

\end{groupplot}
\end{tikzpicture}
\caption{Scaling behavior across configurations for Load, Transform, Embed, Upsert, Total, and Speedup vs NoParallel baseline. 32 workers; embed batch size 64; upsert batch size 256.}
\label{fig:scaling_all}
\end{figure*}



AAFLOW, on the other hand, handles ingestion as a distributed compute graph with non-blocking dataflow scheduling, adaptive micro-batching, and first-class queueing between stages, ensuring that no stage is compelled to wait for another. The empirical results show this shift: (i) Load time collapses from ~4s to ~0.01s, effectively eliminating I/O serialization and making Load constant-time across 1→4096 chunks; (ii) Transform collapses from ~25–26s to sub-second latency, eliminating the global synchronization barrier that dominates stage overlap (e.g., PipelineParallelSync); (iii) Embed time collapses from ~255s to ~0.54s at 4096 chunks, showing near-ideal chunk scaling until micro-batch inference latency limits; and (iv) Upsert scales from ~34.4s to ~4.3s at 4096 chunks, with continuous improvement down to the single-digit node regime due to asynchronous commit buffering and QPS smoothing. Significantly, at 4096 chunks, the total pipeline latency decreases from 298.7s to 5.62s, leading to a 53× end-to-end speedup and continued scaling efficiency beyond the point when generic frameworks usually saturate because to shuffling, memory fragmentation, or tail-delay effects.

The cross-stage queueing discipline and tail-effect suppression necessary for ultra-scale embedding pipelines are not optimized by systems like Spark/Dataproc, Ray, Dask, TF Data, and Triton; instead, they focus on either ETL throughput or model inference throughput. AAFLOW occupies a unique position on the spectrum of systems design: it transforms a throughput-bound workload into a latency-minimal streaming compute graph by completely eliminating barriers rather than overlaying them (as in pipeline parallelism). As far as we are aware, previous ingestion frameworks do not concurrently (i) collapse stage-level latencies across Load/Transform/Embed/Upsert, (ii) maintain near-linear chunk scaling to the multi-thousands in number, and (iii) change the limiting factor from distributed coordination to micro-batch inference latency—a bottleneck profile that differs significantly from that of existing data processing and serving systems.

    




\begin{comment}


\begin{figure}[htpb]
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=3 by 2,
        horizontal sep=1.8cm,
        vertical sep=2.2cm
    },
    ybar,
    ymode=log,
    ymin=1e-3,
    width=5.5cm,
    height=4.5cm,
    bar width=9pt,
    symbolic x coords={NoParallel,ReaderParallel,PipelineParallelSync,AsyncParallelOnly,AgenticDRC},
    xtick=data,
    xticklabel style={rotate=25, anchor=east},
    ymajorgrids=true
]

% 1) Load
\nextgroupplot[
    title={Load (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=gray!70] coordinates {
    (NoParallel,          5.246)
    (ReaderParallel,     32.667)
    (PipelineParallelSync,0.010)
    (AsyncParallelOnly,   0.010)
    (AgenticDRC,          0.010)
};


% 2) Transform
\nextgroupplot[
    title={Transform (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=blue!60] coordinates {
    (NoParallel,          0.127)
    (ReaderParallel,      0.051)
    (PipelineParallelSync,26.945)
    (AsyncParallelOnly,   0.898)
    (AgenticDRC,          0.979)
};

% 3) Embed
\nextgroupplot[
    title={Embed (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=green!60] coordinates {
    (NoParallel,          311.319)
    (ReaderParallel,      311.490)
    (PipelineParallelSync,311.457)
    (AsyncParallelOnly,   10.093)
    (AgenticDRC,          0.737)
};


% 4) Upsert
\nextgroupplot[
    title={Upsert (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=orange!80] coordinates {
    (NoParallel,          43.673)
    (ReaderParallel,      45.712)
    (PipelineParallelSync,46.957)
    (AsyncParallelOnly,   47.489)
    (AgenticDRC,          5.594)
};

% 5) Total time
\nextgroupplot[
    title={Total (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=purple!60] coordinates {
    (NoParallel,          366.789)
    (ReaderParallel,      389.988)
    (PipelineParallelSync,385.447)
    (AsyncParallelOnly,    58.545)
    (AgenticDRC,            7.376)
};

% 6) Speedup vs baseline (NoParallel)
\nextgroupplot[
    title={Speedup vs Baseline},
    ylabel={Speedup ($\times$) (log)}
]
\addplot[fill=teal!60] coordinates {
    (NoParallel,          1.00)
    (ReaderParallel,      0.94)
    (PipelineParallelSync,0.95)
    (AsyncParallelOnly,   6.27)
    (AgenticDRC,         49.73)
};

\end{groupplot}
\end{tikzpicture}

\caption{Per-stage runtime and overall speedup for all configurations. Each subplot shows a separate metric (Load, Transform, Embed, Upsert, Total time, and speedup vs NoParallel baseline) on a logarithmic scale to visualize both large and very small runtimes (e.g., AgenticDRC).}
\label{fig:parallel_3x2_metrics}
\end{figure}


    
\end{comment}


==> tex/Dissertation/AgenticDRC_scaling.tex <==
\subsection{AAFLOW Hybrid Parallel Ingestion Pipeline Benchmarking}

The experimental results demonstrate that AAFLOW outperforms traditional parallelization strategies by restructuring the workload rather than merely accelerating execution. Using a controlled synthetic ingestion setup, we compare multiple configurations, showing that naive parallelism (AsyncParallelOnly, RayDataScalableRAG) yields only modest gains, while asynchronous execution (DaskScalableRAG) significantly reduces runtime by overlapping I/O, transformation, and embedding operations. Across pipeline stages, distinct performance patterns emerge. In the \textit{Load} phase, AAFLOW (0.014 s) achieves better execution time than DaskScalableRAG (0.111 s), indicating that data movement is no longer a bottleneck. In the \textit{Transform} phase, execution times remain similar across approaches, but AAFLOW selectively processes only relevant subsets of data, whereas other methods transform all nodes. The largest gains occur in the \textit{Embed} stage, where DaskScalableRAG reduces latency (1.231 s) through concurrency, while AAFLOW also minimizes computation (1.246 s) by reducing the number and size of embeddings via agentic planning. In the \textit{Upsert} phase, AAFLOW significantly lowers indexing costs (3.024 s) by inserting fewer, higher-value vectors, avoiding redundant storage operations.


\begin{table}[t]
\centering
\caption{Benchmark comparison across parallel configurations (16384 chunks, 1024 files).}
\label{tab:parallel_benchmarks}
\scriptsize
%\setlength{\tabcolsep}{13pt}
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{
    l
    l
    l
    l
    l
    l
    l
}
\toprule
\textbf{Config}
 & {\textbf{Load}}
 & {\textbf{Trans.}}
 & {\textbf{Embed}}
 & {\textbf{Upsert}}
 & {\textbf{Total}}
 & {\textbf{Boost}} \\
 & {(s)} & {(s)} & {(s)} & {(s)} & {(s)} &  \\
\midrule

RayDataScalableRAG  & 2.525   & 0.178        & 0.340    & 6.403     & 9.446  & 1 \\

AsyncParallelOnly   & 1.099   & 0.383        & 1.054    & 1.077     & 3.687    & 2.56  \\

DaskScalableRAG     & 0.409   & 0.189        & 0.444    & 1.946     & 2.988      & 3.16 \\

HigressRAG     & 0.035   & 0.076        & 0.145    & 0.310     & 0.581 & 16.25 \\

\textbf{AAFLOW}     &  0.036   & 0.076  & 0.146   & 0.067  & \textbf{0.340} & \textbf{27.78} \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\scriptsize \textit{AAFLOW vs DaskScalableRAG and HigressRAG, total improvement: $8.78\times$ and $1.70\times$ faster with 16 logical workers}
\end{table}


Overall, AAFLOW achieves up to $10.47\times$ speedup over the baseline and substantially outperforms asynchronous parallelism alone(table-\ref{tab:parallel_benchmarks}). These results demonstrate that while parallelism improves scheduling efficiency, agentic workload reduction fundamentally reshapes the computational cost profile, enabling scalable and efficient RAG ingestion pipelines.

\subsection{Scaling AAFLOW Parallel Ingestion with Multiple Operators}

AAFLOW is designed for model-driven ingestion pipelines, where the critical path spans Load, Transform, Embed, and Upsert operations, unlike traditional ETL or inference-centric systems such as Spark, Ray, Dask, or GPU-based pipelines. While these systems optimize either bulk-synchronous data processing or single-stage throughput, they rely on stage barriers, external coordination, and ad hoc queueing, limiting scalability and increasing latency. In contrast, AAFLOW models ingestion as a distributed, non-blocking compute graph with adaptive micro-batching and cross-stage queueing, eliminating synchronization barriers between stages. This design enables substantial performance improvements across all operations: Load becomes effectively constant-time, Transform reduces from tens of seconds to sub-second latency, Embed scales from hundreds of seconds to sub-second execution, and Upsert achieves significant reductions through asynchronous buffering and smoothed commit rates (Fig. \ref{fig:scaling_all}).

As a result, total pipeline latency decreases from 298.7s to 5.62s at 4096 chunks, achieving over $50\times$ end-to-end speedup while maintaining near-linear scaling (Fig. \ref{fig:scaling_all}). These results demonstrate that AAFLOW shifts the bottleneck from distributed coordination to micro-batch inference latency, fundamentally redefining the performance profile of large-scale RAG ingestion pipelines.


\begin{figure*}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style = {
    group size = 3 by 2,
    horizontal sep = 1.6cm,
    vertical sep = 2.2cm
  },
  width=0.32\linewidth,
  height=0.25\linewidth,
  xmode=log,
  log basis x=2,
  xmin=1, xmax=4096,
  xtick={1,2,4,8,16,32,64,128,256,512,1024,2048,4096},
  xticklabels={1,2,4,8,16,32,64,128,256,512,1024,2048,4096},
  xticklabel style={rotate=90, anchor=east},
  grid=both,
  legend cell align={center},
  legend style={
    font=\scriptsize,
    legend columns=5,
    at={(1.8,1.18)},
    anchor=south,
    draw=none,
    column sep=0.35cm
  },
  xlabel={No of Chunks}
]

% ------------------------------------------------------------------
% 1) LOAD
% ------------------------------------------------------------------
\nextgroupplot[
  title={Load},
  ylabel={Time (s)},
  ymode=log
]

\addlegendentry{NoParallel}
\addlegendentry{ReaderParallel}
\addlegendentry{PipelineParallelSync}
\addlegendentry{AsyncParallelOnly}
\addlegendentry{AAFLOW}

\addplot[red, thick,mark=*] coordinates {
  (1,4.191)(2,4.459)(4,4.31)(8,3.978)
  (16,4.453)(32,4.298)(64,4.521)(128,4.475)
  (256,4.207)(512,4.605)(1024,4.609)(2048,4.443)
  (4096,4.092)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,30.823)(2,30.932)(4,30.661)(8,31.277)
  (16,30.909)(32,31.413)(64,31.452)(128,30.973)
  (256,32.135)(512,32.117)(1024,31.816)(2048,31.45)
  (4096,30.815)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.006)(2,0.006)(4,0.006)(8,0.006)
  (16,0.006)(32,0.006)(64,0.006)(128,0.006)
  (256,0.008)(512,0.008)(1024,0.008)(2048,0.008)
  (4096,0.009)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.006)(2,0.006)(4,0.006)(8,0.006)
  (16,0.006)(32,0.006)(64,0.006)(128,0.006)
  (256,0.006)(512,0.008)(1024,0.008)(2048,0.008)
  (4096,0.009)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.006)(2,0.006)(4,0.006)(8,0.006)
  (16,0.006)(32,0.006)(64,0.006)(128,0.007)
  (256,0.007)(512,0.007)(1024,0.009)(2048,0.008)
  (4096,0.01)
};

% ------------------------------------------------------------------
% 2) TRANSFORM
% ------------------------------------------------------------------
\nextgroupplot[
  title={Transform},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,0.001)(2,0.001)(4,0.001)(8,0.001)
  (16,0.001)(32,0.001)(64,0.001)(128,0.002)
  (256,0.003)(512,0.007)(1024,0.013)(2048,0.022)
  (4096,0.113)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.0)(2,0.0)(4,0.0)(8,0.001)
  (16,0.001)(32,0.001)(64,0.001)(128,0.002)
  (256,0.003)(512,0.005)(1024,0.103)(2048,0.019)
  (4096,0.13)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,25.201)(2,25.043)(4,25.182)(8,24.935)
  (16,24.685)(32,25.628)(64,25.464)(128,25.353)
  (256,25.769)(512,25.367)(1024,25.803)(2048,26.345)
  (4096,26.341)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.247)(2,0.244)(4,0.248)(8,0.257)
  (16,0.248)(32,0.258)(64,0.254)(128,0.281)
  (256,0.283)(512,0.339)(1024,0.392)(2048,0.498)
  (4096,0.678)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.252)(2,0.248)(4,0.247)(8,0.263)
  (16,0.25)(32,0.254)(64,0.265)(128,0.286)
  (256,0.289)(512,0.345)(1024,0.4)(2048,0.614)
  (4096,0.727)
};

% ------------------------------------------------------------------
% 3) EMBED
% ------------------------------------------------------------------
\nextgroupplot[
  title={Embed},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,0.062)(2,0.125)(4,0.249)(8,0.498)
  (16,0.998)(32,1.992)(64,3.984)(128,7.967)
  (256,15.935)(512,31.875)(1024,63.75)(2048,127.59)
  (4096,255.0)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.062)(2,0.125)(4,0.249)(8,0.498)
  (16,0.996)(32,1.992)(64,3.983)(128,7.965)
  (256,15.935)(512,31.876)(1024,63.751)(2048,127.513)
  (4096,255.082)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.062)(2,0.125)(4,0.249)(8,0.498)
  (16,0.996)(32,1.991)(64,3.989)(128,7.966)
  (256,15.934)(512,31.964)(1024,63.752)(2048,127.562)
  (4096,255.063)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.062)(2,0.062)(4,0.063)(8,0.063)
  (16,0.063)(32,0.065)(64,0.129)(128,0.257)
  (256,0.516)(512,1.032)(1024,2.067)(2048,4.139)
  (4096,8.325)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.063)(2,0.063)(4,0.066)(8,0.071)
  (16,0.081)(32,0.101)(64,0.141)(128,0.145)
  (256,0.153)(512,0.17)(1024,0.202)(2048,0.277)
  (4096,0.54)
};

% ------------------------------------------------------------------
% 4) UPSERT
% ------------------------------------------------------------------
\nextgroupplot[
  title={Upsert},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,0.005)(2,0.007)(4,0.01)(8,0.018)
  (16,0.035)(32,0.071)(64,0.152)(128,0.351)
  (256,0.903)(512,2.595)(1024,8.139)(2048,16.688)
  (4096,34.448)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.004)(2,0.006)(4,0.01)(8,0.018)
  (16,0.034)(32,0.073)(64,0.151)(128,0.362)
  (256,0.917)(512,2.687)(1024,8.397)(2048,17.164)
  (4096,35.709)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.003)(2,0.005)(4,0.009)(8,0.017)
  (16,0.033)(32,0.069)(64,0.151)(128,0.366)
  (256,0.955)(512,2.75)(1024,8.618)(2048,17.576)
  (4096,37.311)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.004)(2,0.006)(4,0.011)(8,0.019)
  (16,0.038)(32,0.074)(64,0.167)(128,0.363)
  (256,0.936)(512,2.724)(1024,8.529)(2048,17.573)
  (4096,37.463)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.004)(2,0.005)(4,0.006)(8,0.007)
  (16,0.012)(32,0.021)(64,0.041)(128,0.096)
  (256,0.202)(512,0.439)(1024,0.902)(2048,1.97)
  (4096,4.286)
};

% ------------------------------------------------------------------
% 5) TOTAL
% ------------------------------------------------------------------
\nextgroupplot[
  title={Total},
  ylabel={Time (s)},
  ymode=log
]

\addplot[red, thick,mark=*] coordinates {
  (1,7.971)(2,8.143)(4,9.467)(8,8.582)
  (16,9.329)(32,11.36)(64,15.662)(128,17.829)
  (256,25.68)(512,47.276)(1024,81.662)(2048,155.056)
  (4096,298.708)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,30.895)(2,31.068)(4,30.944)(8,31.799)
  (16,31.945)(32,33.486)(64,35.593)(128,39.307)
  (256,48.998)(512,66.695)(1024,104.082)(2048,176.171)
  (4096,321.797)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,25.278)(2,25.183)(4,25.462)(8,25.46)
  (16,25.726)(32,27.699)(64,29.615)(128,33.697)
  (256,42.673)(512,60.105)(1024,98.202)(2048,171.532)
  (4096,318.787)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,0.34)(2,0.323)(4,0.332)(8,0.349)
  (16,0.36)(32,0.408)(64,0.577)(128,0.913)
  (256,1.748)(512,4.129)(1024,11.037)(2048,22.261)
  (4096,46.528)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,0.329)(2,0.333)(4,0.339)(8,0.353)
  (16,0.353)(32,0.387)(64,0.459)(128,0.555)
  (256,0.679)(512,0.995)(1024,1.545)(2048,2.906)
  (4096,5.624)
};

% ------------------------------------------------------------------
% 6) SPEEDUP VS BASELINE
% ------------------------------------------------------------------
\nextgroupplot[
  title={Speed vs baseline},
  ylabel={Speedup ($\times$)},
  ymin=0
]

\addplot[red, thick,mark=*] coordinates {
  (1,1)(2,1)(4,1)(8,1)
  (16,1)(32,1)(64,1)(128,1)
  (256,1)(512,1)(1024,1)(2048,1)
  (4096,1)
};

\addplot[blue, thick,mark=square*] coordinates {
  (1,0.2580)(2,0.2621)(4,0.3059)(8,0.2699)
  (16,0.2920)(32,0.3392)(64,0.4400)(128,0.4536)
  (256,0.5241)(512,0.7088)(1024,0.7846)(2048,0.8801)
  (4096,0.9282)
};

\addplot[orange,thick,mark=triangle*] coordinates {
  (1,0.3153)(2,0.3234)(4,0.3718)(8,0.3371)
  (16,0.3626)(32,0.4101)(64,0.5289)(128,0.5291)
  (256,0.6018)(512,0.7866)(1024,0.8316)(2048,0.9039)
  (4096,0.9370)
};

\addplot[purple,thick,mark=diamond*] coordinates {
  (1,23.4441)(2,25.2105)(4,28.5151)(8,24.5903)
  (16,25.9139)(32,27.8431)(64,27.1438)(128,19.5279)
  (256,14.6911)(512,11.4497)(1024,7.3989)(2048,6.9654)
  (4096,6.4200)
};

\addplot[green, thick,mark=otimes*] coordinates {
  (1,24.2280)(2,24.4535)(4,27.9263)(8,24.3116)
  (16,26.4278)(32,29.3540)(64,34.1220)(128,32.1243)
  (256,37.8203)(512,47.5136)(1024,52.8557)(2048,53.3572)
  (4096,53.1131)
};

\end{groupplot}
\end{tikzpicture}
\caption{\arupNote{This figure has to be changed due to adding new baseline and experiments} Scaling behavior across configurations for Load, Transform, Embed, Upsert, Total, and Speedup vs. NoParallel baseline. 32 workers; embed batch size 64; upsert batch size 256.}
\label{fig:scaling_all}
\end{figure*}




\begin{comment}


\begin{figure}[htpb]
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=3 by 2,
        horizontal sep=1.8cm,
        vertical sep=2.2cm
    },
    ybar,
    ymode=log,
    ymin=1e-3,
    width=5.5cm,
    height=4.5cm,
    bar width=9pt,
    symbolic x coords={NoParallel,ReaderParallel,PipelineParallelSync,AsyncParallelOnly,AgenticDRC},
    xtick=data,
    xticklabel style={rotate=25, anchor=east},
    ymajorgrids=true
]

% 1) Load
\nextgroupplot[
    title={Load (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=gray!70] coordinates {
    (NoParallel,          5.246)
    (ReaderParallel,     32.667)
    (PipelineParallelSync,0.010)
    (AsyncParallelOnly,   0.010)
    (AgenticDRC,          0.010)
};


% 2) Transform
\nextgroupplot[
    title={Transform (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=blue!60] coordinates {
    (NoParallel,          0.127)
    (ReaderParallel,      0.051)
    (PipelineParallelSync,26.945)
    (AsyncParallelOnly,   0.898)
    (AgenticDRC,          0.979)
};

% 3) Embed
\nextgroupplot[
    title={Embed (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=green!60] coordinates {
    (NoParallel,          311.319)
    (ReaderParallel,      311.490)
    (PipelineParallelSync,311.457)
    (AsyncParallelOnly,   10.093)
    (AgenticDRC,          0.737)
};


% 4) Upsert
\nextgroupplot[
    title={Upsert (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=orange!80] coordinates {
    (NoParallel,          43.673)
    (ReaderParallel,      45.712)
    (PipelineParallelSync,46.957)
    (AsyncParallelOnly,   47.489)
    (AgenticDRC,          5.594)
};

% 5) Total time
\nextgroupplot[
    title={Total (s)},
    ylabel={Seconds (log)}
]
\addplot[fill=purple!60] coordinates {
    (NoParallel,          366.789)
    (ReaderParallel,      389.988)
    (PipelineParallelSync,385.447)
    (AsyncParallelOnly,    58.545)
    (AgenticDRC,            7.376)
};

% 6) Speedup vs baseline (NoParallel)
\nextgroupplot[
    title={Speedup vs Baseline},
    ylabel={Speedup ($\times$) (log)}
]
\addplot[fill=teal!60] coordinates {
    (NoParallel,          1.00)
    (ReaderParallel,      0.94)
    (PipelineParallelSync,0.95)
    (AsyncParallelOnly,   6.27)
    (AgenticDRC,         49.73)
};

\end{groupplot}
\end{tikzpicture}

\caption{Per-stage runtime and overall speedup for all configurations. Each subplot shows a separate metric (Load, Transform, Embed, Upsert, Total time, and speedup vs NoParallel baseline) on a logarithmic scale to visualize both large and very small runtimes (e.g., AgenticDRC).}
\label{fig:parallel_3x2_metrics}
\end{figure}


    
\end{comment}

\subsection{Performance on Semantic Memory Lookup and Hybrid Retrieval}

We compare AAFLOW and HigressRAG \cite{lin2025higress} on semantic cache lookup and hybrid retrieval. The measurements show that semantic cache lookup latency is less AAFLOW, but while raw hybrid retrieval latency is lower for HigressRAG. However, on conversational retrieval tasks where the follow-up query depends on previous context, AAFLOW substantially improves retrieval quality through memory-based query expansion. The benchmark therefore exposes a direct latency--accuracy tradeoff: HigressRAG is better for self-contained low-latency retrieval, while AAFLOW is better for context-dependent retrieval quality.

HigressRAG is treated as a thinner retrieval path derived from the Higress AI gateway abstraction~\cite{higress_repo,higress_cache}. It includes semantic cache lookup, hybrid retrieval, and context assembly without hierarchical memory load/store. AAFLOW uses the same semantic cache and hybrid retrieval primitives, but also augments the query path with hierarchical memory.  This adds latency due to memory operations, but can improve retrieval quality on conversational or underspecified follow-up queries.

To generate latency metrics for each query, the benchmark records:
\begin{itemize}
    \item \texttt{semantic\_cache\_lookup\_ms}: time spent checking the semantic cache,
    \item \texttt{retrieval\_ms}: time spent in hybrid retrieval and context assembly,
    \item \texttt{memory\_load\_ms}: Agentic-only time spent loading hierarchical memory,
    \item \texttt{memory\_store\_ms}: Agentic-only time spent updating memory after answering,
    \item \texttt{total\_ms}: end-to-end latency for the benchmarked scenario.
\end{itemize}

For conversational retrieval, the benchmark reports the following:
\begin{itemize}
\item \texttt{count}: number of retrieval cases evaluated, 
\item \texttt{top1\_accuracy}: fraction of cases where the correct chunk is ranked first.
\begin{equation}
\mathrm{Top1} = \frac{1}{N}\sum_{i=1}^{N}\mathbf{1}[r_i = 1]
\end{equation}
where $r_i$ is the rank of the first correct result for case $i$.
\item \texttt{hit\_at\_k\_accuracy}: fraction of cases where the correct chunk appears in the top-$k$,
\begin{equation}
\mathrm{Hit@}k = \frac{1}{N}\sum_{i=1}^{N}\mathbf{1}[r_i \le k]
\end{equation}
\item \texttt{MRR}: Mean Reciprocal Rank.
\begin{equation}
\mathrm{MRR} = \frac{1}{N}\sum_{i=1}^{N}\frac{1}{r_i}
\end{equation}
If no correct result is found, the reciprocal-rank contribution is treated as $0$.
\end{itemize}


Table~\ref{tab:semantic-cache-fast} summarizes the semantic cache lookup scenario. This run evaluates $1600$ warm-cache lookups per system. Semantic cache lookup is negligible for both systems despite better performance on hybrid retrieval (Table \ref{tab:conv-large}). In both runs, the lookup time is far below one millisecond. The dominant practical result is that both systems achieve a cache hit rate of $1.0$ on the warm cache scenario. The difference in end-to-end total time comes from non-lookup overhead in the benchmark harness rather than the cache similarity search itself.

\begin{table}[!t]
\caption{Semantic Cache Lookup Latency: Large Multicore Run}
\label{tab:semantic-cache-fast}
\centering
\begin{tabular}{lrrrr}
\toprule
System & Count & Hit Rate & Lookup (ms) & Total (ms) \\
\midrule
AAFLOW & 1600 & 1.00 & 0.0008 & 1.3068 \\
HigressRAG & 1600 & 1.00 & 0.0008 & 1.1281 \\
\bottomrule
\end{tabular}
\end{table}




\begin{table}[!t]
\caption{Hybrid Retrieval Latency: Large Multicore Run}
\label{tab:hybrid-fast}
\centering
\begin{tabular}{llllll}
\toprule
System & Count & Retrieval & Mem. & Mem. & Total \\
 &  &  & Load & Store & (ms) \\
\midrule
AAFLOW & 1600 & 3.8031 & 0.4912 & 0.1922 & 6.1202 \\
HigressRAG & 1600 & 2.4470 & 0.0000 & 0.0000 & 4.6329 \\
\bottomrule
\end{tabular}
\end{table}

For hybrid retrieval, Table~\ref{tab:hybrid-fast} reports the same metric after enabling the knowledge cache, and AAFLOW is almost the same as HigressRAG on raw hybrid retrieval latency, despite the overhead of memory load and memory store. In the large-memory configuration, the total time of AAFLOW is 6.1202 ms, which moves closer to HigressRAG (4.6329 ms).


For Conversational Retrieval: Large Run, 
Table~\ref{tab:conv-large} reports retrieval quality from the latest large multicore run. The run sampled $2000$ real source files from \texttt{wikitext2\_train}, requested up to $2000$ conversational cases, and produced $1195$ valid evaluation cases after case construction and filtering.

\begin{table}[!t]
\caption{Conversational Retrieval Quality: Large Multicore Run}
\label{tab:conv-large}
\centering
\begin{tabular}{lrrrr}
\toprule
System & Count & Top-1 & Hit@k & MRR \\
\midrule
AAFLOW & 1195 & 0.9560 & 1.0000 & 0.9730 \\
HigressRAG & 1195 & 0.0010 & 0.9940 & 0.0060 \\
\bottomrule
\end{tabular}
\end{table}

These quality results show where AAFLOW has a clear advantage. On conversational follow-up queries: AAFLOW strongly improves Top-1 ranking, achieves perfect Hit@k in the latest large run and, and greatly improves MRR. The reason is that AAFLOW uses prior-turn context, which acts as memory-based query expansion, while HigressRAG only receives the follow-up query. HigressRAG works a bit better when the query is self-contained, the main objective is minimum latency, and memory augmentation is not required. In that regime, semantic cache lookup is effectively identical, and raw hybrid retrieval latency is lower. AAFLOW is the better choice when the query depends on prior conversation state, the follow-up query is elliptical or underspecified, and retrieval quality matters more than the smallest possible latency.
In that regime, the system pays a bit higher retrieval latency but gains substantially better Top-1, Hit@k, and MRR.



==> tex/Dissertation/BAP_method.tex <==
\subsection{Parallel Processing Models for Ingestion Pipelines}

We consider an ingestion workload of $N$ items processed in batches of size $b$ with up to $P$ parallel workers. The cost of processing a batch is modeled as
\begin{equation}
T_{\text{batch}} = \alpha + \beta b,
\end{equation}
where $\alpha$ denotes fixed per-request overhead and $\beta$ the per-item cost.

\begin{comment}

\subsection{Bulk Synchronous Parallel (BSP)}

BSP executes computation in $S$ synchronized supersteps, each consisting of parallel work, communication, and a barrier. The total cost is
\begin{equation}
T_{\text{BSP}} = \sum_{s=1}^{S} \left(\frac{w_s}{P} + g h_s + L\right),
\end{equation}
where $w_s$ is computation, $h_s$ communication volume, $g$ communication cost, and $L$ barrier latency. While BSP ensures structured execution, the barrier term $L$ introduces synchronization overhead.

    
\end{comment}

\subsection{Ray-Based Execution}

Ray expresses computation as distributed tasks. Its runtime can be approximated as
\begin{equation}
T_{\text{Ray}} \approx \frac{N}{bP}(\alpha_r + \beta_r b) + \sigma_r,
\end{equation}
where $\alpha_r$ captures task scheduling overhead and $\sigma_r$ reflects object-store and coordination costs. Ray provides flexible parallelism but incurs additional runtime overhead per task.

\subsection{Dask-Based Execution}

Dask executes a task graph with explicit dependencies. Its cost is modeled as
\begin{equation}
T_{\text{Dask}} \approx \frac{N}{bP}(\alpha_d + \beta_d b) + \gamma_d,
\end{equation}
where $\alpha_d$ denotes scheduling overhead and $\gamma_d$ captures graph management and communication costs. Dask performs well for coarse-grained workloads but suffers from graph and shuffle overhead at fine granularity.

\subsection{AAFLOW Parallel Batching}

With batching and asynchronous execution, the total runtime is approximated as
\begin{equation}
T_{\text{AAFLOW}} \approx \frac{N}{bP}(\alpha + \beta b)
= \frac{N\alpha}{bP} + \frac{N\beta}{P}.
\end{equation}
This formulation shows that parallelism reduces useful work by a factor of $P$, while batching amortizes overhead by a factor of $b$. Across all models, execution time can be expressed as
\begin{equation}
T \approx \frac{N\beta}{P} + \frac{N\alpha}{bP} + \Omega,
\end{equation}
where $\Omega$ represents framework-specific overhead:
\begin{itemize}
    \item $\Omega \approx 0$ for ideal async batching,
    %\item $\Omega = SL$ for BSP (barriers),
    \item $\Omega = \sigma_r$ for Ray (task/object overhead),
    \item $\Omega = \gamma_d$ for Dask (graph/shuffle overhead).
\end{itemize}

AAFLOW parallel batching minimizes $\Omega$, whereas Ray, and Dask trade additional coordination overhead for structure, scalability, or programmability.

==> tex/Dissertation/conclusion.tex <==

\section{Discussion and Future Experiments}

AAFLOW's parallel execution offers a simple way to increase throughput at first glance: more concurrent requests should, in principle, result in more tokens produced per unit of time. The benchmark results, however, show an unexpected truth: AAFLOW routinely completes generations faster, with lower overall wall-time and higher effective throughput. The way each execution model handles context, scheduling, and cognitive burden is the cause, not the sheer decoding speed. The runtime of AAFLOW incorporates stages of organized reasoning. The approach significantly decreases needless token expansions by letting agents plan ahead, choosing what to obtain, which tools to use, and how to summarize intermediate outcomes. Repeated memory prefill operations, one of the most costly parts of transformer inference, are reduced by bulk planning. Additionally, retrieval-augmented generation is handled more intelligently: AAFLOW recovers just what is pertinent to the current reasoning aim, rather than mindlessly appending copious amounts of contextual input. As a result, the model needs to process fewer tokens on both the input and output sides, which lowers attention overhead. Token budgeting keeps models from overshooting by generating verbose or redundant output, while multi-step scheduling coordinates the transitions between reasoning, retrieval, and production phases to minimize lengthy communication pauses.

In contrast, AAFLOWS reveals inefficiencies that intensify under cognitive workloads. Because concurrent streams frequently lack coordination, individual activities halt on I/O or retrieval, resulting in idle waits. Because there is no common process for determining what information is truly required, parallel workers retrieve overlapping or irrelevant contexts. 
%They often result in partial decodes that increase computational redundancy by neither converging nor reusing KV caches. Even in cases where tasks are semantically related, each stream bears the entire KV creation cost in the absence of common context management. 
Instead of completing the underlying work more quickly, the system frequently overgenerates to fill the pipeline, taking use of parallel slots. As a result, there is a paradoxical situation where the benefits of greater concurrency reduce. So, the comparison shows that increased parallelism does not always equate to increased efficiency. The ability to think before creating is just as important as the ability to create quickly for challenges involving thinking, planning, and retrieval. Instead of only increasing the workload's surface-level parallelism, AAFLOW succeeds by optimizing its cognitive structure.


\textbf{In Future,} we will design the RAG ingestion pipeline experiments to provide a comprehensive and stage-aware evaluation of system performance by explicitly capturing execution time across the Load, Transform, Embed, and Upsert phases of the pipeline. We will further evaluate AAFLOW across multiple vector store backends to understand how storage and indexing characteristics influence end-to-end ingestion performance. To isolate the impact of context management, we will analyze AAFLOW with and without memory-based context loading, along with the impact of using different types of memory, measuring its effect on both latency and stability.


\section{Conclusion}

AAFLOW, a unified distributed runtime that combines cylon, and LlamaIndex into a unified architecture for high-performance, scalable, and repeatable RAG systems, is presented in this paper. AAFLOW offers a deterministic, communication-efficient infrastructure that can handle challenging, multi-agent reasoning tasks, bridging the gap between data-intensive AI workflows and high-performance computing.

AAFLOW achieves up to 8x faster ETL processing than LlamaIndex's default async parallel and Ray parallel ingestion, by demonstrating significant gains in data preparation efficiency and end-to-end RAG pipeline throughput through rigorous performance evaluation. Cylon's high-throughput data operators, Llamaindex's resource-deterministic orchestration, and adaptive agentic retrieval work together to create a synergistic foundation for scalable AI pipelines that preserve speed and reproducibility—two qualities that are frequently at odds in today's large-scale LLM applications. This study reveals a crucial architectural change in AI systems that goes beyond simple performance: modular agentic processes that integrate data engineering, retrieval, and reasoning have replaced monolithic inference models. This progress is embodied in the design of AAFLOW, which supports dynamic, context-aware reasoning at the orchestration layer while permitting deterministic execution at the data layer.

%Future developments in cross-domain reasoning, meta-orchestration across diverse computational environments, and federated agentic workflows can all benefit from the framework. AAFLOW is a major step toward the development of trustworthy, autonomous AI systems that can function effectively in both scientific and enterprise-scale environments by building a scalable and dependable database.


\begin{comment}

\section*{Acknowledgments}
We gratefully acknowledge the support from the Department of Energy and National Science Foundation through DE-SC0023452, NSF 1931512,NSF 2103986, and OAC-2411009 grants. The RADICAL team thanks Andre Merzky and Matteo Turilli for their support and development of RADICAL-Cybertools.
    
\end{comment}





==> tex/Dissertation/design.tex <==
\section{Architectural Design}
\label{sec:design}
Three interconnected obstacles frequently plague traditional RAG architectures: (1) non-deterministic preprocessing; (2) fragmented data orchestration; and (3) static retrieval procedures. In large-scale deployments, these constraints result in uneven embedding spaces, reduced retrieval accuracy, and excessive inference delay. Data preparation in traditional RAG pipelines usually uses sequential Python-based procedures that are unable to efficiently parallelize across big datasets. Semantic drift in vector indices results from the inconsistent generation of embeddings among dispersed nodes. Additionally, additional serialization overhead results from the absence of a common data abstraction across different data formats, which slows down the training and inference phases.
By using distributed determinism and hybrid orchestration, AAFLOW consists of multiple components, including data infrastructure, agentic orchestration, RAG, and a memory module (knowledge cache) shown in Fig.-\ref{fig:aaflow} that directly address these problems.

\begin{figure}[htpb]
    \begin{center}
    \includesvg[width=1.0\linewidth]{Figure/AAFLOW3.svg}
    \caption{End-to-End code flow of AAFLOW with memory operation. The RAG context constructor uses the memory module through the retriever. } 
    \label{fig:aaflow}
    \end{center}
\end{figure}

\subsection{Data Infrastructure}
In order to manage operations like document intake, indexing, and vector embedding creation, efficient Retrieval-Augmented Generation (RAG) systems mainly rely on scalable and high-performance data preparation pipelines. Fundamentally, structured and semi-structured data are represented by a table-based abstraction in Cylon, which allows distant operators to collaboratively manage divided datasets over several processing tiers \cite{widanage2020high}. Large-scale text corpora and embeddings may be separated, processed, and aggregated effectively thanks to this approach, which is essential for creating and maintaining massive RAG knowledge stores. In Fig. \ref{fig:cylon-arch}, cylon's dual-layer interface for Python and C++ guarantees seamless integration with contemporary AI toolchains \cite{alsaadi2025rhapsody}, striking a balance between quick local execution and effective inter-node communication for distributed workflows \cite{cylondoc, merzky2022radical}.

\begin{figure}[htpb]
    \begin{center}
        \includesvg[width=0.7\linewidth]{Figure/cylon-arch.svg}
        \end{center}
        \caption{Cylon Layered Architecture. From the bottom-up view, the Hardware layer is compatible with vendor-based or open-sourced transport layer \cite{perera2023depth}}
    \label{fig:cylon-arch}
\end{figure}

Cylon uses network-level communication primitives based on TCP, InfiniBand, and unified backends like MPI, UCX \cite{shamis2015ucx}, GLOO \cite{gloo:online} and FMI \cite{staylor2025combining} to satisfy the bandwidth and latency requirements of RAG preprocessing (Fig. \ref{fig:cylon-arch}). RAG indexing and embedding generation tasks are dominated by data-intensive distributed operations like shuffle, gather, and reduce, which depend on these communication layers. 
The resulting abstraction reduces I/O overhead and enhances scalability in multi-node environments by supporting high-throughput, communication-aware data movement \cite{shan2022hybrid, perera2023supercharging}.

By offering zero-copy interchange with downstream embedding and vector database systems, Cylon's data model—which is based on the Apache Arrow columnar format—further improves RAG data operations. By facilitating effective feature extraction and vector transformation, this foundation connects deep learning inference with large-scale data preprocessing. Cylon offers the high-performance data foundation needed for scalable, repeatable, and low-latency RAG pipelines running on contemporary HPC and AI infrastructures when included in hybrid frameworks like Deep Radical-Cylon (Deep RC) and RHAPSODY \cite{perera2023depth, alsaadi2025rhapsody}.


    



%\TODO{GREGOR CAME TILL HERE}


\begin{comment}
    
\subsection{Deep Radical-Cylon}

An expansion of Radical-Cylon \cite{sarker2024radical}, Deep Radical-Cylon (Deep RC) is a unified distributed system that integrates Cylon \cite{osti_10634837}, RADICAL-Pilot \cite{radicaldoc}, and contemporary deep learning frameworks through a smooth Python API interface(Fig. \ref{fig:cylon_rp_design}). It makes it possible for large-scale data engineering and AI tasks to be efficiently orchestrated, executed, and communicated across heterogeneous high-performance computing (HPC) environments. Fundamentally, RADICAL-Pilot manages resources and schedules tasks across distributed systems, acting as the execution backbone. A RADICALPilot is used to represent each deep learning or data processing activity.The necessary CPUs, GPUs, and RAM are specified via the TaskDescription object. While the TaskManager assigns Cylon and deep learning tasks to distant nodes \cite{merzky2022radical}, the PilotManager provides the required compute resources. In order to do GLOO/NCCL/MPI operations on these nodes, RemoteAgents dynamically build a hybrid communicator, allowing for concurrent HPC and AI workloads with great communication efficiency.

\begin{figure}[htpb]
    \begin{center}
    \includesvg[width=0.80\linewidth]{Figure/deep-radical-cylon-blk.svg}
    \caption{Deep RC design incorporating Radical-Cylon \cite{sarker2024radical} Architecture with GLOO and NCCL as communication framework. A modular design with dependent components. Segregated independent module with top-down flow from cross-platform to hardware resources. Application pipeline is incorporated with Cylon APIs and PyTorch and TensorFlow with Deep RC Bridge}
    \label{fig:cylon_rp_design}
    \end{center}
\end{figure}

Two interoperability layers are introduced by Deep RC to unify data and resource management: the System Bridge synchronizes execution between Cylon and RADICAL-Pilot \cite{osti_10634837}, and the Data Bridge allows zero-copy data exchange between distributed Cylon dataframes and deep learning tensors (e.g., PyTorch or TensorFlow). This architecture preserves modularity and loose connectivity between components while achieving scalable, deterministic, and high-throughput execution. Deep RC offers a strong foundation for large-scale, repeatable, and communication-efficient agentic AI workflows in both the scientific discovery and enterprise AI domains by fusing resource determinism with high-performance data transfer.
\end{comment}



\begin{comment}
\subsection{Agent Based RAG}
By incorporating external knowledge retrieval processes into the text generation process, Retrieval-Augmented Generation (RAG) \cite{lewis2020retrieval} is a sophisticated natural language processing (NLP) framework that improves the capabilities of large language models (LLMs). RAG provides more precise, current, and contextually appropriate answers by dynamically accessing external data sources rather than depending just on the static knowledge stored during pretraining. Fundamentally, RAG consists of two main parts: \textbf{Retrieval System -}  documents or information from an external knowledge base (such as a vector database, search index, or document storage) are the responsibility of the retrieval system.

\textbf{Generation System –} a large language model (LLM) that creates a logical, contextually grounded response by combining the retrieved data with the user's query. By augmenting "parametric memory" (information stored in model weights) with "non-parametric memory" (knowledge retrieved in real-time), this hybrid approach enables LLMs to overcome its limitations.

RAG uses a series of procedures that combine generation and information retrieval in AWS \cite{aws_rag}. 
\textbf{Query Embedding and Retrieval:} A user's query is first transformed into an embedding, which is a numerical vector representation. The semantic meaning of the question \cite{reimers2019sentencebert} is captured by this embedding. The most semantically related documents or text segments are then found by comparing this vector with pre-stored document embeddings in an external resource, such as a vector database or knowledge index \cite{aws_rag}. 

\textbf{Context Integration:} According to K2view, the original query is then integrated with the obtained context, which could contain pertinent text passages, metadata, or structured data. For the LLM or intelligent agent, this combined input acts as a thorough prompt, guaranteeing that the generated output is both based on recovered evidence and in line with the user's purpose \cite{k2view_rag}. 
\textbf{Response Generation:} In order to generate a human-like, informative, and contextually relevant response, the LLM processes the combined query and context. Both the factual foundation given by the retrieved texts and the linguistic patterns acquired during training serve as guidelines for the generation.

The System Shell Layer, the Prompt Orchestration Layer, and the LLM Inference Core are the three layers that make up systems, as previously discussed \cite{arxiv2508}. The Orchestration Layer can now be managed by frameworks like LangChain \cite{langchain2023} and LangGraph, which allow for conditional logic and persistent state across queries \cite{reddit25}), they present a fresh set of problems with quality control that stem from architectural fragility \cite{arxiv2508}. Because the LLM Inference Core is non-deterministic, it is challenging to forecast or replicate the dynamic execution path that the Orchestration Layer determines. The use of conventional software testing techniques is complicated by this dynamic abstraction layer, necessitating semantic reinterpretation \cite{arxiv2508}.
    
\end{comment}

\subsection{Agent-Based Retrieval-Augmented Generation}
\label{subsec:agent_rag}

Retrieval-Augmented Generation (RAG) enhances large language models (LLMs) by integrating external knowledge retrieval into the generation process, enabling responses that are more accurate, up-to-date, and contextually grounded. Traditional RAG architectures follow a fixed pipeline consisting of retrieval and generation components, where a user query is embedded, matched against a knowledge base, and subsequently used to condition the LLM’s response. While effective, this pipeline assumes a static execution flow and lacks adaptability for complex or multi-step queries \cite{lewis2020retrieval, arxiv2508}. In contrast, \textbf{AAFLOW} introduces an adaptive control mechanism in which an intelligent agent governs the interaction between retrieval and generation. Rather than executing a predefined sequence, the agent dynamically determines when to retrieve, how to reformulate queries, and how to integrate intermediate results. This transforms RAG from a linear pipeline into a decision-driven system capable of iterative reasoning \cite{yao2023react, shinn2023reflexion}.

Formally, given a user query $q$, the agent performs \textit{query interpretation and planning}, where it decides whether retrieval is required and may decompose $q$ into sub-queries $\{q_1, q_2, \dots, q_n\}$. Each sub-query is embedded into a vector representation and used to retrieve relevant documents from an external knowledge base (e.g., a vector database such as ChromaDB \cite{hong2025context, hong2025benchmarking}, FAISS \cite{johnson2019faiss}). Unlike static RAG, the agent can iteratively refine queries based on intermediate retrieval outcomes, enabling multi-hop reasoning and improved recall. The retrieved documents are then processed in a \textit{context integration} stage, where the agent filters, ranks, and aggregates evidence. This step is critical for reducing noise and ensuring that only high-quality, task-relevant information is passed to the LLM. In practice, the agent may also perform additional reasoning operations such as summarization or cross-document synthesis prior to generation. During \textit{response generation}, the LLM produces an output conditioned on both the original query and the curated context. The agent can further introduce feedback loops by validating outputs against retrieved evidence or triggering additional retrieval steps if the response is incomplete or inconsistent. This iterative refinement improves robustness and factual consistency compared to single-pass generation.

%Architecturally, agent-based RAG systems can be decomposed into three layers: (i) a \textit{System Shell Layer} that manages interfaces and tool access, (ii) a \textit{Prompt Orchestration Layer} where the agent resides and controls execution flow, and (iii) the \textit{LLM Inference Core} responsible for generation \cite{arxiv2508}. Modern orchestration frameworks such as LangChain \cite{langchain2023}, LangGraph \cite{langgraph2024}, and LlamaIndex \cite{liu2023llamaindex} enable conditional execution, tool chaining, and persistent state, which are essential for implementing agent-based workflows.

%Despite its advantages, agent-based RAG introduces new challenges. The non-deterministic nature of LLM inference, combined with dynamic agent decision-making, leads to variability in execution paths, complicating reproducibility and debugging. Furthermore, the increased system complexity necessitates new evaluation methodologies, as traditional unit testing is insufficient for capturing semantic correctness and end-to-end behavior \cite{arxiv2508}.

%Overall, agent-based RAG extends conventional RAG by enabling adaptive retrieval, iterative reasoning, and feedback-driven generation, making it well-suited for complex, knowledge-intensive tasks.



\subsection{Agentic Orchestration}
Large-scale, repeatable LLM operations are designed on proposed AAFLOW, which combines Cylon for distributed data preparation and LlamaIndex \cite{liu2023llamaindex} for retrieval orchestration. The framework is built on a two-tier architecture in Fig. \ref{fig:agentic_cylon_design}: (1) the Cylon-powered data engineering layer and (2) the LlamaIndex-managed agentic orchestration layer. 
%The data layer uses distributed Cylon Tables, which use Apache Arrow memory layouts for zero-copy data access, to ingest raw documents from heterogeneous sources (such as relational databases, S3 buckets, and enterprise knowledge bases). The data is subjected to text normalization, token-aware segmentation, and metadata alignment across nodes using Cylon's distributed operators (such as parallel map, join, shuffle, and reduce). After that, each division is vectorized using distributed embedding tasks, which make use of batch processing and GPU acceleration for high throughput. A single schema and consistent alignment with the original document IDs are ensured by materializing the embeddings and related metadata back into Arrow-based vector tables.
LlamaIndex uses the preprocessed and vectorized datasets in the orchestration layer to create hybrid retrieval indices that combine lexical and dense retrieval techniques for adaptive RAG processes. For multi-turn reasoning tasks, LlamaIndex's agentic core offers retrieval hooks and context managers, enabling LLMs to dynamically query pertinent context. Before creating the context window for the downstream LLM inference, LlamaIndex gets the top-k document embeddings via RAG pipelines and re-ranks them using task-specific similarity metrics.

\begin{figure}[htpb]
    \begin{center}
    \includesvg[width=0.8\linewidth]{Figure/Agentic_Cylon1.svg}
    \caption{AAFLOW design incorporating LlamaIndex as an agentic framework. Cylon plays a key role in storing embeddings and data preprocessing. A RAG bridge is used to manage task workflow with LlamaIndex.}
    \label{fig:agentic_cylon_design}
    \end{center}
\end{figure}

\begin{comment}

\begin{figure}[htpb]
    \begin{center}
    \includesvg[width=0.50\linewidth]{Figure/RAG_LamaIdx1.svg}
    \caption{A control flow of agentic cylon with restoring mechanism of context with embeddings.  A CyMEM is used to store and retrieve embedding for LLMs' response with RAG.} 
    \label{fig:rag_cylon_design}
    \end{center}
\end{figure}
    
\end{comment}



\subsection{Memory in agentic RAG: Storing agent state and Intermediate results}
Static retrieval from external knowledge bases is the foundation of traditional RAG systems, which usually use embeddings to retrieve semantically meaningful chunks. However, there is an urgent need for memory modules that store, remember, and dynamically adjust contextual knowledge as LLMs move toward agentic behavior—where they can reason, plan, and interact with tools \cite{karpathy2022agents}. The knowledge (KV) cache and vector store are the foundation for continuity and adaptation in AAFLOW, bridging the gap between short-term interactions and long-term learning (Fig. \ref{fig:aaflow}). In this section, we describe how memory maintains agent state and intermediate findings, connects with retrieval pipelines, and facilitates multi-agent orchestration for planning and reasoning in three important components.

\textbf{Agent State:} An agent may need to monitor prior inquiries, choices, retrievals, tool calls, and results in multi-turn dialogues or workflows. This state (such as vector embeddings of previous interactions or summaries of previous reasoning) can be kept in a memory module. Memory changes with users and gets better over time because it records user preferences, past questions, choices, and mistakes \cite{intelvector}.

\textbf{Intermediate Results:} 
The documents that were retrieved, the chunks that were used, the embeddings that were created, and the portions of the context that were put into the model are examples of intermediate results during a retrieval-generation cycle. These outcomes can be stored in a memory module so that subsequent retrievals or reasoning stages don't have to start from scratch. For instance, a system explained how continuity is enhanced when a retrieval module and a memory module are combined. Two-Way Retrieval Both the retrieval module (for static knowledge) and the memory module (for historical/contextual data in knowledge cache) are queried by the system \cite{karpathy2022agents}.

\textbf{Contextual Continuity: } Context and personalization are supported via memory modules. They enable agents to recall things like "the earlier plan failed because of missing data" or "the user emphasized safety compliance in the last exchange" and modify subsequent retrievals accordingly. This implies that retrieval is dependent on a history of interactions in addition to the current query.

\begin{comment}
    


\subsection{Architectural Overview }
A memory-augmented Agentic RAG system's architecture is based on the idea of adaptive reasoning via perseverance. Agentic RAG preserves permanent cognitive traces—records of inquiries, reasoning, and outcomes—across interactions, in contrast to traditional RAG systems that reset state after each inference. Agents are able to coordinate intricate operations, recall previous reasoning, and improve replies thanks to this persistence. Three complementary layers make up the architecture in Fig. \ref{fig:cymem_design}:

\textbf{Retrieval Layer: } Access to static external knowledge sources, such as databases, vector indices, and structured documents, is controlled by this layer. It carries out indexing, embedding, and similarity search functions. The layer facilitates distributed scaling via frameworks like Cylon or FAISS and is in charge of effective retrieval utilizing dense vector representations.
Providing factual context is the Retrieval Layer's main duty. Nevertheless, it also engages in dynamic interaction with the Memory Layer in Agentic RAG, giving context or previous results back into the retrieval query formulation. For instance, re-ranking or query reformulation may be guided by feedback if the agent previously retrieved certain documents that produced less-than-ideal results.

\textbf{Agentic Orchestration Layer:} 
This layer serves as the framework's cognitive center. It is made up of several cooperating agents, like: \texttt{Retrieval Agent:} carries out memory and document retrieval. \texttt{Reasoning Agent:} combines and evaluates context from multiple sources. \texttt{Response Agent:} generates the finished user-facing output, which may be enhanced with references or supporting data. Coordination and non-redundant reasoning are ensured by each agent communicating via a common memory substrate. The decision graph, which keeps track of which agents completed whose tasks, their outputs, and dependencies, is maintained by the orchestration layer. Replay, debugging, and performance monitoring are made possible by this.

\textbf{Memory Layer:} As a bidirectional bridge, the Memory Layer receives data from agents and provides past state in response to new inquiries. The Memory Layer holds dynamic context, such as agent state, intermediate results, user preferences, and outcomes, in contrast to the Retrieval Layer, which stores static domain information. It guarantees consistency and offers the framework for flexible behavior throughout sessions.


\begin{figure}[htpb]
    \begin{center}
    \includesvg[width=0.8\linewidth]{Figure/cymem.svg}
    \caption{Block Diagram for the involvement of memory in the orchestration and context generation layer in CyMEM!}
    \label{fig:cymem_design}
    \end{center}
\end{figure}
\end{comment}

==> tex/Dissertation/evaluation.tex <==
\section{Performance Evaluation} 

\subsection{Experimental Setup} 
We put up weak and strong scalability utilizing the \texttt{bii-gpu} queue with 37 cores per node and 4 A100s GPUs using UVA Rivanna HPC~\cite{rivanna_2023}. The goal is to assess AAFLOW's effectiveness when doing multitask LLM inferences and compare it to other agentic frameworks, like Langchain\cite{langchain2023}, LangGraph \cite{langgraph2024}, and CreaAI. Two metrics will be measured: DRC overheads and throughputs, as well as total and average execution time. The Total Execution Time shows how much time AAFLOW spent using the computational resources to carry out the LLM inference and data pretreatment activities. The overheads show how long it takes DRC to (i) deserialize the task object and (ii) build the \texttt{Communicator} with N rankings and send it to the tasks. The average time required by all N levels is represented by the average execution time. N ranks are required for each agentic job, with a maximum of 10,000 inferences per rank. 

A series of tests was carried out on heterogeneous high-performance computing (HPC) and multi-GPU clusters to evaluate the resilience and performance of the suggested Agentic RAG Framework. The studies focused on three aspects: (1) distributed preprocessing throughput, (2) retrieval latency and accuracy, and (3) scalability and repeatability under dynamic workloads. They mainly evaluated the framework against conventional RAG and standard LLM inference pipelines. Using Cylon for distributed ETL and embedding generation and LlamaIndex for resource orchestration, the system was implemented on HPC systems.


\begin{table}[!t]
\caption{RAG Pipeline Benchmark on 12800 tokens generated from 200 Documents with Tuned Streaming AAFLOW. All metrics are measured in seconds}
\label{tab:framework-rag-results}
\centering
\begin{tabular}{lllllll}
\toprule
Framework  & Load & Trans & Tokens/s & Embed  & Upsert & Total \\
\midrule
LangChain & 0.0214 & 0.0060 & 10149.01 & 0.5810 & 0.1687 & 2.0383 \\
LangGraph  & 0.0205 & 0.0054 & 10152.91 & 0.5665 & 0.1705 & 2.0237 \\
CrewAI & 0.0187 & 0.0051 & 10151.89 & 0.5671 & 0.1933 & 2.0450 \\
AutoGen & 0.0183 & 0.0056 & 10151.79 & 0.5581 & 0.1667 & 2.0096 \\
AAFLOW & 0.0201 & 0.0064 & 10149.13 & 0.2797 & 0.1605 & 1.7279 \\
\bottomrule
\end{tabular}
\end{table}




\begin{comment}
\subsection{Distributed Preprocessing and ETL Throughput} 

Data preparation and embedding creation, which are usually carried either sequentially or with coarse-grained parallelism, are two of the main bottlenecks in traditional RAG systems. The suggested system achieves near-linear scaling in ETL activities including document chunking, tokenization, and vector embedding by utilizing Cylon's distributed dataframe and Arrow-based memory architecture. Preprocessing throughput increased by about 6\% with 10\% less latencies on an 8-node cluster (Fig.- \ref{fig:cylon_latency_throughput}) compared to the baseline RAG pipeline implemented with Python multiprocessing. Using Cylon operators, we have introduced document load, cleaning, and chunk creation to the RAG pipeline.  Cylon's capacity to reduce serialization overhead and preserve memory locality during transformation and shuffle operations is the source of this gain.






\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style={
    group size=1 by 2,
    vertical sep=1.0cm
  },
  ybar,
  width=\columnwidth,
  height=0.55\columnwidth,
  bar width=5pt,
  ymode=log,
  symbolic x coords={Docs,Chunks},
  xtick=data,
  xticklabel style={font=\footnotesize},
  tick label style={font=\footnotesize},
  ymajorgrids=true,
  legend style={
    at={(0.5,1.2)},
    anchor=south,
    legend columns=2,
    font=\footnotesize
  },
]

% ---------------- Latency Panel ----------------
\nextgroupplot[
  title={Latency},
  title style={font=\footnotesize},
  ylabel={Seconds (log scale)},
  ylabel style={font=\footnotesize},
]
\addplot[fill=red] coordinates {
  (Docs,   2.07115e-05)
  (Chunks, 6.53323e-07)
};
\addplot[fill=green] coordinates {
  (Docs,   1.69046e-05)
  (Chunks, 5.48730e-07)
};
\legend{Agentic DRC, Async Parallel}

% ---------------- Throughput Panel ----------------
\nextgroupplot[
  title={Throughput},
  title style={font=\footnotesize},
  ylabel={Tokens/s (log scale)},
  ylabel style={font=\footnotesize},
]
\addplot[fill=red] coordinates {
  (Docs,   4.82822e+04)
  (Chunks, 1.43064e+06)
};
\addplot[fill=green] coordinates {
  (Docs,   5.28275e+04)
  (Chunks, 1.60231e+06)
};

\end{groupplot}
\end{tikzpicture}

\caption{Latency and throughput comparison for Docs and Chunks workloads with and without Cylon acceleration. Log-scale emphasizes magnitude differences and relative performance improvement.}
\label{fig:cylon_latency_throughput}
\end{figure}

Furthermore, concurrent execution of embedding generation and index construction across worker nodes was made possible by RADICAL-Pilot's dynamic task scheduling. Through pilot-level telemetry, this will decrease idle time and increase resource use efficiency. RADICALPilot.TaskDescription's structured description of ETL tasks will enable exact control over GPU and CPU allocations, guaranteeing deterministic and repeatable execution over several runs.

\end{comment}

\subsection{Framework Benchmarking for RAG Pipeline}
AAFLOW records the lowest total time, $1.7279$~s. The strongest non-Agentic baseline is AutoGen at $2.0096$~s (Table \ref{tab:framework-rag-results}). The end-to-end speedup is therefore approximately
\begin{equation}
\frac{2.0096}{1.7279} \approx 1.16\times
\end{equation}
relative to the best non-Agentic result in this fair-parallelism experiment. This is a much smaller gap than in the default benchmark mode because all frameworks now share the same concurrency cap and batch sizes. After tuning the overlap implementation with persistent executors and dedicated embed/upsert worker pools, the larger I/O-bound workload shows an improvement for AAFLOW. 
\par
The remaining measurable advantage for AAFLOW appears in the ingest-heavy stages (embed and upsert, (Fig \ref{fig:fair-stage-times}) and (Table \ref{tab:framework-rag-results})):
\begin{equation}
\texttt{embed\_s}_{\mathrm{AAFLOW}} = 0.2797\ \mathrm{s}
\end{equation}
\begin{equation}
\texttt{upsert\_s}_{\mathrm{AAFLOW}} = 0.1605\ \mathrm{s}
\end{equation}
\begin{itemize}
    \item \texttt{embed\_s}: $0.2797$~s vs. $0.5581$--$0.5810$~s for the other frameworks,
    \item \texttt{upsert\_s}: $0.1605$~s vs. $0.1667$--$0.1933$~s for the other frameworks.
\end{itemize}
These differences persist after normalizing worker count and batch size. In the best run, the dominant gain comes from the streaming bounded-queue Agentic path with separate embed/upsert worker pools and bulk upsert coalescing. The largest improvement is on embedding, where dedicated embed workers remove the previous fair-path bottleneck.

AAFLOW reaches $10149.1307$ tokens/s, while the next best result is LangGraph at $10152.9193$ tokens/s and CrewAI at $10151.8926$ tokens/s. The throughput values are effectively identical across frameworks once the same parallelism budget is enforced. This result is expected. Because every framework uses the same worker cap and the same generation batch size. The dominant throughput difference from the default mode therefore disappears. AAFLOW retains the best total time after introducing a streaming bounded-queue path, separate embed/upsert worker pools, and bulk upsert coalescing (Fig \ref{fig:fair-stage-times}). The default-mode advantage of AAFLOW is therefore partly due to better batching and concurrency design, and partly due to lower remaining framework overhead.
The tuned overlap implementation helps only on a larger or more I/O-bound workload; stage overlap is not automatically beneficial unless stage latency is large enough to amortize coordination cost.





\begin{figure}[!t]
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=9pt,
    width=\columnwidth,
    height=0.58\columnwidth,
    ylabel={Seconds},
    symbolic x coords={LangChain,LangGraph,CrewAI,AutoGen,AAFLOW},
    xtick=data,
    x tick label style={rotate=25,anchor=east, font=\scriptsize},
    %legend style={at={(0.5,1.18)},anchor=south,legend columns=2},
    legend style={
    font=\scriptsize,
    legend columns=5,
    at={(0.5,1.1)},
    anchor=south,
    draw=none,
    column sep=0.35cm
  },
    ymin=0,
]
\addplot coordinates {(LangChain,0.0214) (LangGraph,0.0205) (CrewAI,0.0187) (AutoGen,0.0183) (AAFLOW,0.0201)};
\addplot coordinates {(LangChain,0.0060) (LangGraph,0.0054) (CrewAI,0.0051) (AutoGen,0.0056) (AAFLOW,0.0064)};
\addplot coordinates {(LangChain,0.5810) (LangGraph,0.5665) (CrewAI,0.5671) (AutoGen,0.5581) (AAFLOW,0.2797)};
\addplot coordinates {(LangChain,0.1687) (LangGraph,0.1705) (CrewAI,0.1933) (AutoGen,0.1667) (AAFLOW,0.1605)};
\legend{Load,Transform,Embed,Upsert}
\end{axis}
\end{tikzpicture}
\caption{Framework benchmarking in each vital stage in the RAG pipeline under equal parallelism. AAFLOW beats all frameworks in two vital stages(embed and upsert)}
\label{fig:fair-stage-times}
\end{figure}

\begin{comment}

\subsection{Retrieval Latency and Context Adaptation}

In retrieval experiments using LamaIndex’s agentic retriever, which dynamically selects data sources based on LLM reasoning feedback, the proposed architecture demonstrated substantial gains in both retrieval accuracy and inference latency. Compared to a static FAISS-based retriever, the agentic RAG framework achieved a 23\% reduction in mean retrieval latency and a 17\% improvement in top-k retrieval precision across benchmark datasets (e.g., PubMedQA and WikiText).

This gain can be attributed to two key design decisions: (1) adaptive retrieval strategies, where the LLM’s chain-of-thought or reasoning trace influences query reformulation and ranking order, and (2) Arrow-backed in-memory communication between Cylon and LamaIndex, eliminating redundant deserialization. The integration with RADICAL-Pilot ensures that high-priority retrieval operations receive dedicated compute resources during multi-agent inference sessions, minimizing queuing delays and improving throughput.  

\subsection{Scalability and Reproducibility}

Scalability tests showed that the framework maintained consistent performance up to 128 concurrent nodes without degradation in throughput or retrieval accuracy \cite{johnson2019faiss}. The multi-node communicator management implemented in RADICAL-Pilot allowed efficient orchestration of concurrent distributed operators (e.g., shuffle, reduce, gather) used during RAG preprocessing and embedding refresh. Importantly, the framework exhibited reproducible embedding consistency across distributed environments—where embedding vector drift between independent runs dropped from 2.7\% (baseline) to 0.4\% (proposed), as measured via cosine distance metrics.

Moreover, reproducibility under dynamic workloads—where resources were scaled elastically—remained intact due to the deterministic nature of task allocation and the use of consistent random seeds across distributed ranks. This property is essential for scientific and industrial RAG pipelines, where traceability and explainability are as critical as performance.

\subsection{End-to-End System Efficiency}

End-to-end evaluations integrating data ingestion, preprocessing, retrieval, and inference demonstrated an overall 2.9× improvement in system-level efficiency compared to standard RAG pipelines. The hybrid orchestration of Cylon + RADICAL-Pilot not only reduced end-to-end latency but also provided fine-grained control over resource binding, resulting in predictable and explainable performance profiles.

Collectively, these results confirm that the proposed Agentic RAG Framework successfully addresses the major inefficiencies of current LLM retrieval architectures—providing a scalable, reproducible, and semantically consistent approach to distributed reasoning and adaptive context management.

\section{Discussion and Future Work} 

The integration of Cylon, LamaIndex, and RADICAL-Pilot within the Agentic RAG Framework demonstrates that distributed data preprocessing, adaptive retrieval, and dynamic orchestration can coexist within a unified architecture for large-scale LLM applications. The empirical findings highlight the significant efficiency gains achievable through deterministic ETL pipelines and context-aware retrieval mechanisms. However, several important challenges remain—particularly in scalability, generalization, and cross-domain adaptability—that open pathways for future investigation.

\subsection{Interpretability and Adaptive Control}

One of the emerging frontiers is the interpretability of agentic retrieval behavior. While the current system employs adaptive retrieval through LamaIndex’s agentic reasoning layer, the decision-making process behind query reformulation and context ranking is often opaque. Future work will explore explainable retrieval controllers that trace decision logic, providing insights into why specific context sources were selected. Integrating reinforcement learning from human feedback (RLHF) or self-corrective retrieval mechanisms could further enhance interpretability while ensuring alignment with user intent and factual consistency.

\subsection{Federated and Cross-Domain Data Orchestration}

The present framework primarily targets HPC-based distributed infrastructures; however, many enterprise and research use cases involve federated or hybrid data environments spread across multiple security domains. Extending Cylon’s distributed ETL layer to operate over federated learning settings—where data remains decentralized but feature spaces must be harmonized—represents a crucial next step. Incorporating privacy-preserving protocols such as differential privacy or secure multiparty computation (SMPC) would enable broader adoption in sensitive data contexts, including healthcare and finance. Moreover, expanding the System Bridge abstraction to support multi-cloud orchestration could allow RADICAL-Pilot to dynamically allocate resources between cloud and HPC nodes while preserving reproducibility guarantees.

\subsection{Integration with Vector Databases and Knowledge Graphs}

Although the current implementation relies on LamaIndex’s in-memory retrieval subsystem, future iterations aim to integrate distributed vector databases such as Milvus, Pinecone, or FAISS-GPU to support petabyte-scale retrieval. Such integration will enable the agentic RAG to operate on knowledge graphs and structured enterprise data, extending its reasoning capability beyond unstructured text. Embedding synchronization between the Cylon ETL layer and external vector databases will also be optimized through Arrow Flight RPC, ensuring zero-copy data interchange and consistent vector space alignment across distributed environments.

\subsection{Real-Time Adaptive Inference and Feedback Loops}

Another critical research trajectory involves enabling real-time feedback loops where the agentic retriever dynamically adjusts its context window and reasoning scope during ongoing inference. Coupling LamaIndex’s agent layer with low-latency telemetry streams from RADICAL-Pilot could allow inference-time adaptation to resource availability or contextual novelty. This would create self-regulating agentic pipelines capable of reasoning under uncertainty, resource constraints, or evolving data distributions—moving toward a new class of autonomous reasoning systems for HPC and AI research.

\subsection{Theoretical Advancements and Benchmarks}

While empirical evaluations confirm the system’s scalability and reproducibility, further theoretical analysis is required to establish optimal bounds for communication complexity, embedding drift, and retrieval convergence under distributed operations. Developing a standardized Agentic RAG Benchmark Suite—covering metrics such as semantic stability, resource elasticity, and retrieval precision under varying loads—will provide a rigorous foundation for comparative evaluation against future architectures. Additionally, leveraging graph-based task scheduling models could improve reasoning efficiency by reducing redundant dependency resolution between distributed tasks.

\subsection{Toward a Unified Agentic-HPC Ecosystem}

Ultimately, the convergence of agentic AI frameworks and HPC middleware offers a promising pathway toward a Unified Agentic-HPC Ecosystem, where distributed AI workflows are treated as dynamic, self-optimizing processes. Future research will explore meta-orchestration, where multiple agentic subsystems—such as retrieval, summarization, and decision agents—operate under a shared control policy managed by RADICAL-Pilot. This paradigm could enable large-scale multi-agent collaboration with adaptive data routing and workload balancing across heterogeneous compute environments.

In summary, the proposed method establishes the foundation for scalable, adaptive, and reproducible RAG systems that bridge HPC and AI research. By integrating deterministic data engineering (Cylon), adaptive retrieval (LamaIndex), and dynamic orchestration (RADICAL-Pilot), the proposed framework not only mitigates the inefficiencies of current LLM pipelines but also opens new directions in distributed reasoning, interpretability, and self-organizing AI infrastructure.
\end{comment}


==> tex/Dissertation/implementation.tex <==

\section{Implementation}

Cylon ensures deterministic and reproducible preprocessing by parallelizing tokenization, chunking, and embedding within a unified Arrow-based memory model, eliminating nondeterminism in multi-threaded ETL pipelines. In parallel, LlamaIndex introduces an agentic retrieval layer that dynamically adapts search and ranking strategies based on the LLM’s reasoning state and contextual history. Leveraging Cylon’s distributed communication and Arrow-based data transfer reduces serialization overhead, enabling efficient embedding generation, faster time-to-context, and near-real-time index updates. Together, these components form a scalable, adaptive RAG pipeline that improves retrieval accuracy while maintaining transparency and consistent performance (Fig. \ref{fig:aaflow}).


\subsection{Data Processing Layer: Distributed ETL, Embedding and Retrieval Infrastructure}
The RAG pipeline's high-performance data processing activities are supported by the Cylon distributed DataFrame engine. It supports partitioned datasets and group communication via UCX, Gloo, or MPI, enabling effective ETL (Extract, Transform, Load) activities over several nodes. By eliminating I/O and serialization inefficiencies, Cylon's interface with Apache Arrow enables zero-copy data movement between data processing and deep learning modules. This approach facilitates distributed embedding generation with fast throughput and little communication overhead when paired with PyTorch's DataLoader.
Depending on deployment limitations, models from the Sentence-Transformers or OpenAI API are used to compute embeddings. After being normalized, these embeddings are kept in a distributed vector database like ChromaDB \cite{smith2024evaluating, hong2025benchmarking} FAISS \cite{johnson2019faiss} or Pinecone \cite{pinecone2023}. We implement FAISS in AAFLOW.  Because FAISS offers indexing structures (FlatIP, HNSW, IVF) that are geared for high recall and cosine similarity. Dual FAISS indices—one for static knowledge and one for long-term memory embeddings—are used to carry out memory retrieval queries. A retrieval agent uses a weighted scoring system to combine and rank the findings. 

\begin{comment}

\subsection{Agentic Layer and Orchestration}

LlamaIndex, LangGraph, or personalized agent controllers are used to implement the agentic layer. Every agent (Retrieval, Reasoning, Response) functions as a modular Python process that communicates via message queues (like Redis or Ray) or shared memory. Reasoning chains may be traced because agent decisions are recorded as nodes in a decision graph \cite{langchain2023}.

LlamaIndex manages orchestration across dispersed systems to guarantee deterministic execution and resource repeatability. Allocating resources and sending out agentic tasks with exact scheduling control, it offers a task-based abstraction. A scheduler optionally controls distributed embedding and indexing tasks, requiring predictable execution patterns across nodes to preserve performance consistency and experimental repeatability. Because of this connectivity, the framework can handle scalable data ingestion for corpora larger than terabytes, incremental index changes, and low-latency retrieval. Furthermore, serialization overhead between Cylon and LlamaIndex is reduced by using Arrow as an intermediary memory protocol, allowing retrieval indices to be updated almost instantly. The end product is an end-to-end agentic RAG architecture that addresses major drawbacks of conventional RAG pipelines, including non-deterministic data preprocessing, inconsistent embeddings, and delayed index refreshes, while combining distributed data processing, retrieval orchestration, and contextual augmentation for LLMs.

    
\end{comment}

\begin{comment}

\subsection{Memory Management System and Learning Pipeline}

Both persistent vector stores (LTM) and in-memory caches (STM) are included into the memory system. Redis or Arrow tables are used to implement STM for low-latency lookups. FAISS indices serialized to disk or cloud storage are used by LTM(Fig. \ref{fig:cymem_flow}). Reconstructing agent behavior across sessions is made possible by the storage of episodic memory entries in a Parquet-based knowledge log.

\textbf{Short-Term Memory (STM) : } A temporary buffer is provided by short-term memory. Within an active interaction window or session, it maintains state, which usually includes: 1) The current query and its sub-queries. 2) The relevancy scores of the retrieved documents. 3) Tool invocation records or steps in agentic reasoning. Arrow tables or Redis are used to implement STM as a fast-access cache or an in-memory vector store. Low-latency access and quick read/write are supported. To prevent memory saturation, STM entries may be condensed or summarized into long-term memory after the session is over.

\begin{lstlisting}[language=python]
short_term_memory = {
    "query": "Explain distributed ETL in Cylon",
    "retrieved_docs": [
        {"title": "Cylon Overview", "relevance": 0.92},
        {"title": "Apache Arrow for ETL", "relevance": 0.85}
    ],
    "embedding": [0.33, 0.71, 0.25, 0.48],
    "reasoning_trace": "Cylon uses Arrow for in-memory communication.",
    "intermediate_output": "Compare Arrow vs Spark performance."
}
\end{lstlisting}
All retrieved passages and similarity scores are stored in STM by the Retrieval Agent. In order to synthesize context, the Reasoning Agent consumes STM entries. The resulting summaries or conclusions are updated in STM by the Response Agent. After the work is completed, STM can be compiled and stored in LTM. Consider STM to be the RAG system's RAM; it is quick, erratic, and cleared at the end of the session.

\textbf{Long-Term Memory (LTM) : }
Durable knowledge is persistently stored in long-term memory. Semantically encoded representations of previous sessions, such as outcome metadata, model-generated insights, and user interaction history, are stored. Contextual retrieval that changes according on user experience is made possible by LTM's capability for vectorized search over historical embeddings. Usually, FAISS, Pinecone, or Milvus support LTM. In order to preserve scalability, it also allows for periodic summarizing and pruning, which condenses unnecessary items into higher-level semantic groupings.

\begin{lstlisting}[language=python]
long_term_memory.add(
    embedding=model.encode("Cylon distributed ETL optimization"),
    metadata={
        "user": "ishan",
        "session_id": "2025-10-29-001",
        "summary": "Compared Cylon vs Spark for distributed ETL",
        "outcome": "Cylon achieved 2x throughput",
        "feedback": "Highly relevant and accurate"
    }
)

\end{lstlisting}

STM entries are condensed into brief summaries following an engagement. These summaries are kept in LTM and embedded as semantic vectors. In subsequent sessions, the Retrieval Agent retrieves previous results or insights by querying both the static knowledge base and LTM. Using this remembered context, the Reasoning Agent may modify its behavior, such as favoring Cylon-based responses if previous runs supported them. The next query concerning "distributed ETL optimization" automatically pulls this information from LTM, directing reasoning, if the user had previously asked "Compare Dask and Cylon for ETL" and the system had determined that "Cylon performs better due to Arrow integration." LTM preserves experience and enhances reasoning over time, much like a hard drive for the agent's brain.

\textbf{Episodic Memory (EM) : } High-level narratives of interactions—"episodes" that capture questions, logic, and outcomes in a single sequence—are stored in episodic memory. Semantic linkages between turns are captured by encoding each episode into embeddings. By improving reasoning consistency, EM enables agents to discover patterns like typical query types or efficient retrieval techniques.
Agents can compare new tasks to previous processes and choose the best course of action by using episodic memory as the foundation for meta-reasoning.

A reinforcement layer keeps an eye on query results, user interactions, and agent performance in order to close the feedback loop. It uses contrastive fine-tuning of encoders or incremental retraining to update memory embeddings on a regular basis. Continuous learning is made possible by this adaptive process, in which the memory changes in tandem with the model.

\begin{lstlisting}[language=python]
episodic_memory.append({
    "episode_id": "E2025-10-29-Session001",
    "sequence": [
        {"query": "What is distributed ETL?", "result": "Definition retrieved"},
        {"query": "Explain Cylon's ETL design", "result": "Arrow integration noted"},
        {"query": "Compare Cylon vs Spark", "result": "Cylon 2x faster"}
    ],
    "summary": "Discovered Cylon's performance advantage through Arrow-based ETL",
    "embedding": model.encode("Distributed ETL - Cylon vs Spark study")
})
\end{lstlisting}

During multi-turn interactions, every reasoning step is recorded by the Orchestration Layer. A summary embedding of the complete episode is produced after the session is finished. Future inquiries can retrieve context at the episodic level, such as full successful thought chains. The system may plan complicated activities by reusing episodic patterns (e.g., "use previous time's data preparation method"). Similar to autobiographical memory, episodic memory recalls how the system made decisions, succeeded, or failed in the past.

    
\end{comment}

\subsection{Information Flow in the Memory-Enhanced RAG Pipeline}

The memory-enhanced RAG pipeline operates as a closed-loop system that integrates query understanding, dual retrieval, reasoning, and continuous memory updates. User queries are embedded into vector representations while the memory layer is simultaneously consulted to identify similar past interactions, enabling reuse of prior results and faster inference. The system employs a dual retrieval mechanism, combining knowledge retrieval from a static vector store with memory retrieval of historical context, thereby unifying factual grounding with experiential learning.

The retrieved information is synthesized into a composite context window, where an agent performs reasoning through dynamic planning or structured prompting, while intermediate states are recorded for traceability. Following response generation, the system updates multiple memory layers, including short-term logs, structured summaries, and compressed embeddings stored in long-term memory. This persistent feedback loop allows the system to adapt over time by refining retrieval strategies, optimizing prompts, and incorporating feedback from both successful and unsuccessful outcomes, ultimately improving performance, consistency, and contextual awareness.

\begin{figure}[htpb]
    \begin{center}
        \includesvg[width=0.9\linewidth]{Figure/Advanced_Async_PP2.svg}
        \end{center}
        \caption{Advanced Async with Parallel Pipeline of AAFLOW. With batching to measure execution time. BE = Size of the batch embeddings; BU = Size of the upsert batching. $T_{Total} = Load\ Time + Transform\ Time(t_1 + t_2) + Index\ Time$}
    \label{fig:async_pp}
\end{figure}

\begin{comment}
To observe how STM, LTM, and EM interact, let's replicate a single RAG cycle. "Assess how Cylon enhances distributed ETL efficiency in comparison to Spark." \textbf{In Retrieval Layer →} retrieves Spark and Cylon docs. \textbf{In STM →} keeps temporary reasoning notes, embeddings, and retrieved documents. \textbf{In Reasoning Agent →} compares architectures using STM and produces the intermediate result "Cylon employs zero-copy Arrow." \textbf{Again in Response Agent →} Generates final summary. \textbf{In LTM →} contains metadata about "Cylon's ETL efficiency advantage" and condensed vector embedding. \textbf{Within EM →} keeps track of all the questions, steps in the reasoning process, and conclusions. The next time a user inquires, "What framework is appropriate for Arrow-based ETL?" the agent collects the following information to better comprehend the CyMEM: \textbf{From STM (if in same session):}  Previous partial results. \textbf{From LTM:} The stored performance comparison. \textbf{From EM:} the order in which the conclusion was reached.  The model may reply more quickly and accurately by avoiding unnecessary thinking thanks to its multi-level recall.
    
\end{comment}
\subsection{AAFLOW's Hybrid Asynchronous Parallel Pipeline}

AAFLOW introduces a hybrid asynchronous parallel pipeline built on LlamaIndex ingestion with adaptive resource allocation and bulk embedding generation. By combining parallel batching with optimized upsert operations to the FAISS vector store, the pipeline reduces I/O overhead and improves end-to-end performance (Fig. \ref{fig:async_pp}). A controlled synthetic data generation setup ensures fair benchmarking across configurations by maintaining consistent corpus size, node distribution, and chunk structure.

The pipeline consists of modular stages, including data loading (synchronous or parallel), transformation via a delimiter-based splitter, embedding generation using a deterministic latency-aware model, and vector indexing using FAISS with both flat and sharded backends \cite{pinecone_vector_indexes}. Asynchronous execution and batching are leveraged to simulate realistic large-scale embedding workloads while maintaining reproducibility. Performance is evaluated through detailed stage-wise timing, including load, transform, embedding, indexing, and total execution time, enabling systematic comparison of parallelization strategies.


==> tex/Dissertation/intro.tex <==
\section{Introduction}\label{sec:introduction}

Monolithic models have given way to "Agentic Workflows," which are intricate software systems that use retrieval augmentation, multi-turn interactions, and tool utilization to complete complex tasks \cite{arxiv2508}.  The effectiveness of the underlying data infrastructure is crucial to the usefulness and dependability of these workflows, particularly in knowledge-intensive fields like scientific discovery. However, the shift to sophisticated, integrated AI pipelines reveals two basic architectural flaws in the present industry-standard frameworks.
First, ineffective data processing is the cause of the \textbf{Bottleneck Challenge}. Integrating extensive, domain-specific knowledge sources is necessary for Retrieval-Augmented Generation (RAG) \cite{ibm25}. High-throughput data engineering operations like chunking, indexing, and creating huge vector embeddings are all part of this process \cite{intelvector}. These Extract, Transform, Load (ETL) pipelines result in considerable overheads when using typical distributed data systems because of data transport, serialization charges, and fragmented architectures \cite{llamaindex25}. For example, although functional, frameworks like as Dask and Spark diverge greatly at high parallelisms and show clear restrictions in communication-bound tasks, suggesting profound structural challenges \cite{arxiv2406}. In addition, performance and generality of Dataflow depend on having the right primitives/operators; out-of-distribution pipelines may require manual operator authoring\cite{liang2025dataflow}. Second, the intrinsic features of LLM applications—non-determinism, dynamism, and context dependence—are the foundation of the \textbf{Reliability Challenge} \cite{arxiv2508}. These characteristics make reproducibility and quality assurance more difficult, which are critical for reliable AI and scientific computing \cite{arxiv2509}. High-level orchestration frameworks that are now in use, like LangChain, provide flexibility but frequently function as black-box abstractions that impede thorough performance validation and system debugging \cite{arxiv2508}. Scaling costs and development time are only made worse by a fragmented RAG pipeline that depends on several point solutions for storage, embedding, and retrieval \cite{llamaindex25}. 


The fundamental issue is the mismatch between the requirement for repeatable computational execution of each module in the agentic pipeline and the dynamic, LLM-driven execution flow with respect to access of the index vector DB and back-and-forth memory access for updating context  \cite{arxiv2509}. The guarantee of repeatability is seriously jeopardized if the LLM (the agent) controls the execution environment for tasks (like sentence splitting, token text splitting, embedding generation, data retrieval, or training synchronization). However, RAG systems rely on quick retrieval from large knowledge libraries \cite{ibm25}.  
%The ETL procedures needed for indexing, sentence splitting, token text splitting, and vector embedding creation frequently control this retrieval's performance \cite{intelvector}.  
Scaling these procedures frequently results in extremely fragmented architectural solutions, requiring coordination between several services for data storage, splitting, embedding creation, and retrieval. This significantly raises scaling costs and overall complexity \cite{llamaindex25}. RAG's performance barrier is essentially a data engineering problem: executing quick similarity searches on enormous datasets of high-dimensional vector embeddings \cite{rishabh25}.
%Systems that can sustain high throughput in communication-intensive distributed operations are needed for these data processing jobs.
Significant scaling constraints in these communication-heavy scenarios are shown by analysis of well-known Python-native distributed systems, like Dask and Spark. %These engines have extremely little scalability for GroupBy, despite their excellent scalability for operations like Join and Sort \cite{researchgate24}. 
More importantly, both Dask and Spark diverge considerably at larger parallelisms when exposed to communication-bound tasks using smaller partition sizes transmitted across the same number of workers (e.g., a 100 million-row test case) \cite{researchgate24}. 
The RAG indexing bottleneck is defined as instability that occurs precisely when maximum data movement is needed, and this divergence validates deep, fundamental limits in their underlying communication frameworks. Because of the I/O-bound instability of their backend data pipelines, the observed fragility in high-level LLM applications \cite{arxiv2508} is essentially execution workflow rather than just a semantic issue of prompt engineering. This architectural instability that depends on execution workflow at the data and communication layers must be fixed before a system may scale agentic operations.

As a solution, we provide \textbf{AAFLOW}, a unified, heterogeneous distributed runtime system that smoothly combines multi-agent execution with high-performance data engineering. It is made up of several parts that work together harmoniously to create an end-to-end pipeline. A paradigm that distinguishes between resource and execution management and the logical flow of the program addresses the issues mentioned above. The AAFLOW supports large-scale, repeatable LLM procedures with distributed preprocessing and intelligent retrieval. It has three primary layers: \textbf{Data Engineering Layer (Cylon)} uses Apache Arrow to handle data input from many sources, such as documents, databases, or cloud storage, into distributed tables for quick, zero-copy access. 
In order to extract metadata, create embeddings, and obtain the knowledge graph, Cylon applies normalization, segmentation, sentence splitting, token text splitting, and metadata alignment in simultaneous operations like map, join, and reduce. Using a multi-tiered memory layer, \textbf{Agentic Orchestration Layer (LlamaIndex)} controls information retrieval and coordination. Between agents and the continuing context of the system, the memory layer functions as a two-way conduit. When fresh inputs or queries are received in memory, it provides pertinent historical data in addition to gathering and storing information created by agents.   \textbf{The Memory Layer} guarantees continuity between sessions by preserving this live environment, allowing agents to learn from previous encounters and eventually display adaptive, context-aware behavior. It essentially acts as the framework's cognitive foundation, supporting memory-driven reasoning and tailored answers. To guarantee effective, high-throughput performance, each data division is finally converted into embeddings using distributed, accelerated batch processing. 


Additionally, AAFLOW uses customized asynchronous parallel processing on top of the LlamaIndex ingestion pipeline. It makes use of task-based resource orchestration on multiple modules. All jobs are carried out as independent black boxes in each module\cite{arxiv2105}. AAFLOW's parallel workflow divides the acquisition of resources from their utilization by abstracting them as a single entity. Groups of tasks (workloads) are described and submitted for execution using a "batch-like" approach in the transform, embed, and upserting stages. Bypassing the slow, parallel ingestion for each unit of the upserting and embedding stage, AAFLOW reduces the number of write operations on vector DB, along with the bulk use of embedding to build the index with the highest concurrency allowed by the acquired resources. Deterministic execution routes for computational activities are ensured by this division of responsibilities between resource and execution management, offering the architectural stability required for handling dynamic, high-level agent logic. It provides the foundation for scalable and repeatable agentic processes by removing I/O and serialization bottlenecks through the use of high-speed communication framework and a single data plane. Here are the contributions:

\begin{enumerate}
    \item \textbf{Systematic Architectural Evaluation:} The article offers a thorough examination of the performance divergence and architectural fragility found in popular distributed dataframe implementations and agentic orchestration layers \cite{arxiv2508}. 
    \item \textbf{Unified Architectural Design:} The entire AAFLOW architecture is described, including the unique \textbf{Agent Bridge} required to provide execution synchronization between memory and LlamaIndex, distributed data retrieval with parallel operation, and zero-copy embedding transfer. 
    \item \textbf{Resource Determinism:} The system shows how the asynchronous parallel batching of AAFLOW guarantees deterministic, high-concurrency task execution by substituting explicit resource control for non-deterministic execution dependency, which is essential for creating dependable Agentic execution systems. 
    \item \textbf{Quantitative Validation:} AAFLOW's improved data preprocessing performance is confirmed by extensive strong and weak scaling benchmarks, which also show notable end-to-end acceleration in agentic pipelines and effective memory retrieval. %\cite{researchgate24}. 
\end{enumerate}





==> tex/Dissertation/method.tex <==

\section{Memory Model for Agentic RAG}

The memory-augmented agentic RAG system is described as a recurrent process that develops via a series of interactions indexed by $t$. (1) memory-conditioned query encoding, (2) multi-source retrieval, (3) agent status update, and (4) memory write operations into short-term, long-term, and episodic memory modules make up each phase.

\subsection{Notation}

\begin{equation}
M_t = \big(M_t^{S},\, M_t^{L},\, M_t^{E}\big).
\label{eq:memory_state}
\end{equation}
corresponding to short-term memory (STM), long-term memory (LTM), and episodic memory (EM), respectively.

We define two encoder functions:
\begin{itemize}
    \item $f_{\mathrm{enc}}(\cdot)$: encodes queries and agent inputs,
    \item $f_{\mathrm{mem}}(\cdot)$: encodes memory entries for retrieval.
\end{itemize}

Similarity between vectors is denoted by $\mathrm{sim}(\cdot,\cdot)$.

\subsection{Memory-Conditioned Query Encoding}

Given the input $x_t$ and the previous memory state $M_{t-1}$, we compute a memory-conditioned query embedding:
\begin{equation}
z_t = f_{\mathrm{enc}}\big(x_t,\, M_{t-1}\big).
\label{eq:query_embedding}
\end{equation}

\subsection{Retrieval from Knowledge Base, STM, and LTM}

Let $\mathcal{D} = \{d_i\}$ be an external knowledge base with embeddings $v_i = f_{\mathrm{mem}}(d_i)$. The retrieval score for each document is

\begin{equation}
s_i^{(K)} = \mathrm{sim}(z_t, v_i),
\label{eq:kb_similarity}
\end{equation}

The top-$k$ retrieved knowledge items form

\begin{equation}
C_t^{(K)} = 
\mathrm{TopK}\big(\{d_i\}, \{s_i^{(K)}\}, k\big).
\label{eq:kb_retrieval}
\end{equation}

Short-term memory contains entries $e_j^{S}$ with embeddings
$u_j^{S} = f_{\mathrm{mem}}(e_j^{S})$. Retrieval scores:

\begin{equation}
s_j^{(S)} = \mathrm{sim}(z_t, u_j^{S}),
\label{eq:stm_similarity}
\end{equation}

\begin{equation}
C_t^{(S)} =
\mathrm{TopK}(\{e_j^{S}\}, \{s_j^{(S)}\}, k_S).
\label{eq:stm_retrieval}
\end{equation}

Long-term memory contains persistent entries $e_k^{L}$ with embeddings $u_k^{L} = f_{\mathrm{mem}}(e_k^{L})$. Retrieval scores:

\begin{equation}
s_k^{(L)} = \mathrm{sim}(z_t, u_k^{L}),
\label{eq:ltm_similarity}
\end{equation}
\begin{equation}
C_t^{(L)} =
\mathrm{TopK}(\{e_k^{L}\}, \{s_k^{(L)}\}, k_L).
\label{eq:ltm_retrieval}
\end{equation}

The fused retrieved context is:
\begin{equation}
C_t = \mathrm{Fuse}
\big(C_t^{(K)},\, C_t^{(S)},\, C_t^{(L)}\big).
\label{eq:fused_context}
\end{equation}

where $\mathrm{Fuse}(\cdot)$ denotes concatenation, weighted re-ranking, or a learned attention-based mixing function.

\subsection{Agent State Update}

Given the previous hidden state, current input, and retrieved context, the agent updates its internal state:

\begin{equation}
h_t = f_{\mathrm{agent}}(h_{t-1}, x_t, C_t),
\label{eq:agent_state_update}
\end{equation}

and produces an output:

\begin{equation}
y_t = g_{\mathrm{agent}}(h_t, C_t).
\label{eq:agent_output}
\end{equation}

\subsection{Memory Write Operations}

We define candidate memory writes:
\begin{align}
\tilde{m}_t^{S} &= f_{w}^{S}(h_t, y_t, C_t),
\label{eq:stm_write_candidate} \\
\tilde{m}_t^{L} &= f_{w}^{L}(h_t, y_t, C_t, r_t),
\label{eq:ltm_write_candidate} \\
\tilde{m}_t^{E} &= f_{w}^{E}(h_t, y_t, C_{1:t}).
\label{eq:em_write_candidate}
\end{align}

where $r_t$ is optional feedback and $C_{1:t}$ is the context history.

Memory write gates are defined as:
\begin{align}
\alpha_t^{S} &= \sigma(W_S h_t + b_S),
\label{eq:stm_gate} \\
\alpha_t^{L} &= \sigma(W_L [h_t; r_t] + b_L),
\label{eq:ltm_gate} \\
\alpha_t^{E} &= \sigma(W_E h_t + b_E).
\label{eq:em_gate}
\end{align}

with $\sigma$ the sigmoid function.

\subsubsection{Short-Term Memory Update}

Short-term memory is a bounded buffer of size $N_S$:

\begin{equation}
M_t^{S} =
\mathrm{Truncate}\Big(
M_{t-1}^{S} \cup \{\alpha_t^{S} \tilde{m}_t^{S}\},\, N_S
\Big).
\label{eq:stm_update}
\end{equation}

\subsubsection{Long-Term Memory Update}

Long-term memory performs conditional writes based on a threshold $\tau_L$:

\begin{equation}
M_t^{L} =
M_{t-1}^{L} \cup 
\Big\{
\mathbb{I}[\alpha_t^{L} > \tau_L]\, \tilde{m}_t^{L}
\Big\}.
\label{eq:ltm_update}
\end{equation}

\subsubsection{Episodic Memory Update}

At the end of an episode (interaction sequence $1 \ldots T$), we compute an episodic summary:

\begin{equation}
\tilde{e} =
f_{\mathrm{episodic}}\big(h_{1:T},\, y_{1:T},\, C_{1:T}\big),
\label{eq:episodic_summary}
\end{equation}

and update EM:

\begin{equation}
M_T^{E} =
M_{T-1}^{E} \cup \{\alpha_T^{E}\tilde{e}\}.
\label{eq:episodic_update}
\end{equation}

\subsection{Full Memory-Aware Update}

The complete update for step $t$ is:
\begin{align}
z_t &= f_{\mathrm{enc}}(x_t, M_{t-1}), 
\tag{\ref{eq:query_embedding}} \\
C_t &= \mathrm{Fuse}(C_t^{(K)}, C_t^{(S)}, C_t^{(L)}),
\tag{\ref{eq:fused_context}} \\
h_t &= f_{\mathrm{agent}}(h_{t-1}, x_t, C_t),
\tag{\ref{eq:agent_state_update}} \\
y_t &= g_{\mathrm{agent}}(h_t, C_t),
\tag{\ref{eq:agent_output}} \\
M_t^{S} &= \mathrm{STM\_update}(M_{t-1}^{S}, \tilde{m}_t^{S}, \alpha_t^{S}),
\tag{\ref{eq:stm_update}} \\
M_t^{L} &= \mathrm{LTM\_update}(M_{t-1}^{L}, \tilde{m}_t^{L}, \alpha_t^{L}),
\tag{\ref{eq:ltm_update}} \\
M_t^{E} &= \mathrm{EM\_update}(M_{t-1}^{E}, \tilde{m}_t^{E}, \alpha_t^{E}).
\tag{\ref{eq:episodic_update}}
\end{align}

\begin{comment}


\subsection{Algorithm Pseudocode (STM/LTM/EM Retrieval and Update)}
The proposed Deep RC-enabled Agentic RAG architecture's basic operational workflow is formalized by the Memory-Aware Retrieval and Update Algorithm. The approach creates a fused contextual representation for agentic reasoning at each timestep by performing memory-conditioned query encoding and tri-source retrieval from the static knowledge base, short-term memory (STM), and long-term memory (LTM). A recurrent decision function updates the agent state, producing outputs that could be multi-step plans, tool invocations, or natural-language responses.Then, via controlled insertion, selective persistence, and episode-level summarization, a hierarchical write mechanism updates STM, LTM, and episodic memory (EM). The complete algorithm ensures repeatable, high-throughput execution even in multi-agent deployments by integrating distributed ETL (by Cylon), deterministic resource scheduling (with LlamaIndex), and zero-copy Arrow-based data flow (via Deep RC). In addition to offering a mathematically based paradigm for scalable, memory-augmented agentic AI systems, this organized process permits continuous learning, context retention, and dynamic adaptability across interactions—properties not achievable in traditional, stateless RAG pipelines.

 \begin{figure}[htpb]
    \centering
    \begin{tikzpicture}[
        >=Latex,
        node distance=1.4cm and 1.8cm,
        box/.style={draw, rounded corners, align=center, minimum width=2.7cm, minimum height=1cm},
        smallbox/.style={draw, rounded corners, align=center, minimum width=2.2cm, minimum height=0.8cm},
        arrow/.style={->, thick}
    ]

    % Top: User + Embedding
    \node[box] (user) {User Query\\$q_t$};
    \node[box, below=of user] (emb) {Encoder\\$z_t = f_{\mathrm{enc}}(x_t, M_{t-1})$};

    % Middle: Agentic core
    \node[box, below=of emb] (agent) {Agentic Core\\$h_t, y_t$};

    % Bottom: KB + infra
    \node[box, below=of agent, xshift=-2.8cm] (kb) {Knowledge Base\\Vector Store $\mathcal{D}$};
    \node[box, below=of agent, xshift=1.8cm] (infra) {Infrastructure\\Cylon / FAISS};

    % Memory block on the right
    \node[box, right=3.2cm of agent] (mem) {Memory Layer};
    \node[smallbox, above=0.4cm of mem] (stm) {STM\\$M_t^{S}$};
    \node[smallbox, below=0.0cm of mem] (ltm) {LTM\\$M_t^{L}$};
    \node[smallbox, below=0.4cm of ltm] (em)  {EM\\$M_t^{E}$};

    % Arrows top-down
    \draw[arrow] (user) -- node[right]{input $x_t$} (emb);
    \draw[arrow] (emb) -- node[left]{query embedding $z_t$} (agent);

    % Retrieval arrows
    \draw[arrow] (agent.south) to[bend right=-15] (kb.east);
    \draw[arrow] (kb.north) to[bend left=15] node[pos=0.9, left]{\small $C_t^{(K)}$} (agent.west);

    % Memory retrieval arrows
    \draw[arrow] (agent.east) -- node[above]{retrieve} (mem.west);
    \draw[arrow] (stm.west) -- ++(-1.0,0) |- node[pos=0.15, right]{\small $C_t^{(S)}$} (agent.north);
    \draw[arrow] (ltm.west) -- ++(-1.0,0) |- node[pos=0.2, right]{\small $C_t^{(L)}$} (agent.north);
    \draw[arrow] (em.west)  -- ++(-1.0,0) |- node[pos=-0.15, right]{\small $C_t^{(E)}$} (agent.south east);

    % Write-back arrows
    \draw[arrow] (agent.east) to[bend left=15] node[above]{write} (stm.north west);
    \draw[arrow] (agent.east) to[bend left=5]  node[midway,above]{write} (ltm.west);
    \draw[arrow] (agent.east) to[bend right=15] node[pos=0.6, left]{episode} (em.north west);

    % Infra arrows
    \draw[arrow] (infra.north) -- (agent.south east);
    \draw[arrow] (infra.west) to[bend right=-25] (kb.south);

    \end{tikzpicture}
    \caption{System-level memory architecture for an agentic RAG system. The agentic core retrieves from both the external knowledge base and multi-tier memory (STM, LTM, EM), and writes back state and summaries after each interaction.}
    \label{fig:memory_architecture}
\end{figure}

\begin{algorithm}[htpb]
\caption{Memory-Aware Retrieval and Update in Agentic RAG}
\label{alg:memory_rag}
\begin{algorithmic}[1]
    \Require Input $x_t$, previous memory $M_{t-1} = (M_{t-1}^{S}, M_{t-1}^{L}, M_{t-1}^{E})$
    \Ensure Output $y_t$, updated memory $M_t$
    
    \State $z_t \gets f_{\mathrm{enc}}(x_t, M_{t-1})$ 
        \Comment{memory-conditioned encoding}
    
    \State $C_t^{(K)} \gets \textsc{RetrieveFromKB}(z_t)$
    \State $C_t^{(S)} \gets \textsc{RetrieveFromSTM}(z_t, M_{t-1}^{S})$
    \State $C_t^{(L)} \gets \textsc{RetrieveFromLTM}(z_t, M_{t-1}^{L})$
    
    \State $C_t \gets \mathrm{Fuse}(C_t^{(K)}, C_t^{(S)}, C_t^{(L)})$
    
    \State $h_t \gets f_{\mathrm{agent}}(h_{t-1}, x_t, C_t)$
    \State $y_t \gets g_{\mathrm{agent}}(h_t, C_t)$
    
    \State $(\tilde{m}_t^{S}, \tilde{m}_t^{L}, \tilde{m}_t^{E}) \gets 
            f_{w}^{S,L,E}(h_t, y_t, C_t)$
    
    \State $(\alpha_t^{S}, \alpha_t^{L}, \alpha_t^{E}) \gets 
            \sigma(W h_t + b)$
    
    \State $M_t^{S} \gets 
            \mathrm{Truncate}\big(M_{t-1}^{S} \cup \{\alpha_t^{S} \tilde{m}_t^{S}\}, N_S\big)$
    
    \If{$\alpha_t^{L} > \tau_L$}
        \State $M_t^{L} \gets M_{t-1}^{L} \cup \{\tilde{m}_t^{L}\}$
    \Else
        \State $M_t^{L} \gets M_{t-1}^{L}$
    \EndIf
    
    \If{$t$ is end-of-episode}
        \State $\tilde{e} \gets f_{\mathrm{episodic}}(h_{1:T}, y_{1:T}, C_{1:T})$
        \State $M_t^{E} \gets M_{t-1}^{E} \cup \{\alpha_T^{E}\tilde{e}\}$
    \Else
        \State $M_t^{E} \gets M_{t-1}^{E}$
    \EndIf
    
    \State \Return $y_t, (M_t^{S}, M_t^{L}, M_t^{E})$
\end{algorithmic}
\end{algorithm}

%\section{Algorithm Description}

The proposed \textit{Memory-Aware Retrieval and Update Algorithm} defines the core workflow of the Deep~RC–enabled Agentic RAG system. It governs how inputs are encoded, how multi-source retrieval occurs, how the agent performs reasoning,
and how hierarchical memory is updated. The algorithm proceeds through four stages: memory-conditioned encoding, multi-source retrieval, agentic reasoning, and hierarchical memory updates.

\subsubsection{Memory-Conditioned Encoding}
At timestep $t$, the system receives input $x_t$ and the previous memory state
$M_{t-1} = (M_{t-1}^{S}, M_{t-1}^{L}, M_{t-1}^{E})$.
We compute a memory-conditioned embedding via
\begin{equation}
    z_t = f_{\mathrm{enc}}(x_t, M_{t-1}),
    \label{eq:query_embedding}
\end{equation}
which incorporates short-term, long-term, and episodic information. This enhances contextual continuity compared to stateless RAG systems.


\subsubsection{Multi-Source Retrieval}
Retrieval is performed from three sources:  
the static knowledge base (KB), short-term memory (STM), and long-term memory (LTM). For the KB, similarity scores (e.g., cosine similarity) are computed as
\begin{equation}
    s_i^{(K)} = \mathrm{sim}(z_t, v_i),
    \label{eq:kb_similarity}
\end{equation}
and the top-$k$ retrieved elements are selected:
\begin{equation}
    C_t^{(K)} = \mathrm{TopK}(d_i, s_i^{(K)}, k).
    \label{eq:kb_retrieval}
\end{equation}

STM retrieval parallels this:
\begin{equation}
    s_j^{(S)} = \mathrm{sim}(z_t, u_j^{S}),
    \label{eq:stm_similarity}
\end{equation}
\begin{equation}
    C_t^{(S)} = \mathrm{TopK}(e_j^{S}, s_j^{(S)}, k_S).
    \label{eq:stm_retrieval}
\end{equation}

Similarly for LTM:
\begin{equation}
    s_k^{(L)} = \mathrm{sim}(z_t, u_k^{L}),
    \label{eq:ltm_similarity}
\end{equation}
\begin{equation}
    C_t^{(L)} = \mathrm{TopK}(e_k^{L}, s_k^{(L)}, k_L).
    \label{eq:ltm_retrieval}
\end{equation}

All retrieved signals are fused into a unified representation:
\begin{equation}
    C_t = \mathrm{Fuse}(C_t^{(K)}, C_t^{(S)}, C_t^{(L)}).
    \label{eq:fused_context}
\end{equation}

\subsubsection{Agentic Reasoning and Output Generation}

The fused context drives the agentic controller. The internal agent state evolves according to
\begin{equation}
    h_t = f_{\mathrm{agent}}(h_{t-1}, x_t, C_t),
    \label{eq:agent_state_update}
\end{equation}
and agent output is generated via
\begin{equation}
    y_t = g_{\mathrm{agent}}(h_t, C_t).
    \label{eq:agent_output}
\end{equation}

\subsubsection{Hierarchical Memory Updates}

Candidate memory entries are produced by:
\begin{equation}
    (\tilde{m}_t^{S}, \tilde{m}_t^{L}, \tilde{m}_t^{E})
    = f_{w}(h_t, y_t, C_t).
    \label{eq:stm_write_candidate}
\end{equation}

Memory write gates are computed via:
\begin{equation}
    (\alpha_t^{S}, \alpha_t^{L}, \alpha_t^{E})
    = \sigma(W h_t + b).
    \label{eq:stm_gate}
\end{equation}

STM is updated with gated insertion and truncation:
\beg




\subsection{Unified Training Objective}

We optimize a joint objective that couples task performance with memory quality.Let $\mathcal{L}_{\mathrm{task}}$ denote the primary task loss (e.g., cross-entropy over next-token predictions or answer correctness). We define a retrieval loss
$\mathcal{L}_{\mathrm{ret}}$ and a memory regularization loss
$\mathcal{L}_{\mathrm{mem}}$.

\paragraph{Retrieval Loss.}
For a query embedding $z_t$ and a set of relevant memory or document entries $\mathcal{R}_t$, we enforce that relevant items have higher similarity than non-relevant items:
\begin{equation}
\mathcal{L}_{\mathrm{ret}} =
- \sum_{t} \log 
\frac{\sum_{e \in \mathcal{R}_t} 
    \exp(\mathrm{sim}(z_t, f_{\mathrm{mem}}(e)) / \tau)}
{\sum_{e' \in \mathcal{N}_t}
    \exp(\mathrm{sim}(z_t, f_{\mathrm{mem}}(e')) / \tau)},
\label{eq:retrieval_loss}
\end{equation}
where $\mathcal{N}_t$ includes both relevant and negative entries and $\tau > 0$ is a temperature.

\paragraph{Memory Regularization.}
We constrain write gates to avoid pathological behaviors such as saturating writes or vanishing usage of memory. We use:
\begin{equation}
\mathcal{L}_{\mathrm{mem}} =
\sum_t \big(
\lambda_S \, \alpha_t^{S}(1 - \alpha_t^{S}) +
\lambda_L \, \alpha_t^{L}(1 - \alpha_t^{L}) +
\lambda_E \, \alpha_t^{E}(1 - \alpha_t^{E})
\big),
\label{eq:memory_reg}
\end{equation}
which encourages gate values to avoid extremes of $0$ or $1$.

\paragraph{Total Objective.}
The overall objective is:
\begin{equation}
\mathcal{L} =
\mathcal{L}_{\mathrm{task}} +
\beta_{\mathrm{ret}} \, \mathcal{L}_{\mathrm{ret}} +
\beta_{\mathrm{mem}} \, \mathcal{L}_{\mathrm{mem}},
\label{eq:total_loss}
\end{equation}
where $\beta_{\mathrm{ret}}$ and $\beta_{\mathrm{mem}}$ control the strength of retrieval alignment and memory regularization, respectively.

\subsection{Stability of Memory Updates}

We briefly discuss conditions under which the proposed memory update rules yield a stable evolution of the memory state.

\begin{lemma}[Boundedness of Short-Term Memory]
Assume that (i) each short-term write candidate $\tilde{m}_t^{S}$ has bounded
norm, i.e., $\|\tilde{m}_t^{S}\|_2 \leq C_S$ for all $t$, and
(ii) the buffer size $N_S$ is finite. Then the STM sequence
$\{M_t^{S}\}_{t \geq 0}$ remains bounded.
\end{lemma}

\begin{proof}[Sketch]
At each step, STM is updated via
\[
M_t^{S} = \mathrm{Truncate}\big(M_{t-1}^{S} \cup \{\alpha_t^{S}\tilde{m}_t^{S}\}, N_S\big),
\]
with $\alpha_t^{S} \in [0,1]$. Truncation enforces that the number of stored entries never exceeds $N_S$, and each stored vector has norm at most $C_S$. Hence the STM state can be viewed as an element of a finite product of bounded sets, and is therefore bounded.
\end{proof}

\begin{lemma}[Controlled Growth of Long-Term Memory]
Assume that (i) the LTM write gate satisfies
$\alpha_t^{L} \in [0,1]$ for all $t$, (ii) the write threshold
$\tau_L \in (0,1)$, and (iii) for each $t$ the probability that
$\alpha_t^{L} > \tau_L$ is bounded by $p < 1$. Then the expected size of
$M_t^{L}$ grows at most linearly with $t$ and can be further controlled via down-sampling or periodic pruning.
\end{lemma}

\begin{proof}[Sketch]
By definition,
\[
M_t^{L} = M_{t-1}^{L} \cup 
\Big\{\mathbb{I}[\alpha_t^{L} > \tau_L] \tilde{m}_t^{L}\Big\}.
\]
Taking expectations yields
$\mathbb{E}[|M_t^{L}|] \leq \mathbb{E}[|M_{t-1}^{L}|] + p$,
which unrolls to
$\mathbb{E}[|M_t^{L}|] \leq |M_0^{L}| + p t$.
Thus the memory size is at most linear in $t$ in expectation, and pruning or compaction can ensure practical boundedness.
\end{proof}

\begin{lemma}[Stability of Retrieval Scores]
Assume that all embeddings are $\ell_2$-normalized and that
$\mathrm{sim}(\cdot,\cdot)$ is the dot product. Then for any query embedding $z_t$, all retrieval scores lie in $[-1,1]$ and are therefore uniformly bounded.
\end{lemma}

\begin{proof}[Sketch]
If $\|z_t\|_2 = \|v\|_2 = 1$, then
$\mathrm{sim}(z_t, v) = z_t^\top v \in [-1,1]$ by the Cauchy-Schwarz inequality.
Thus similarity scores used in retrieval and training losses (e.g., in Eq.~\eqref{eq:retrieval_loss}) are uniformly bounded.
\end{proof}

\noindent
Together, these lemmas indicate that, under mild assumptions on gating, thresholding, and normalization, the memory dynamics do not diverge pathologically. In practice, additional mechanisms such as episodic summarization and reservoir sampling further improve stability and scalability.

\subsection{Complexity Analysis}

We briefly summarize the asymptotic complexity of one memory-aware RAG step.

Let $d$ be the embedding dimension, $N_K$ the number of indexed knowledge entries, $N_S$ the STM size, and $N_L$ the LTM size.

\paragraph{Encoding.}
Computing $z_t = f_{\mathrm{enc}}(x_t, M_{t-1})$ has cost
$O(d \cdot L_x)$, where $L_x$ is the effective token length of the input. For transformer-based encoders this is typically
$O(L_x^2 d)$, but we treat it as $O(E)$ for brevity.

\paragraph{Retrieval.}
For an exact dense vector search:
\begin{itemize}
    \item Knowledge base retrieval:
    $O(N_K d)$ to compute all dot products.
    \item STM retrieval:
    $O(N_S d)$.
    \item LTM retrieval:
    $O(N_L d)$.
\end{itemize}
Using approximate nearest neighbor indices (e.g., FAISS IVF/HNSW), the expected cost reduces to $O(\log N_K \cdot d)$ and similarly for LTM.

\paragraph{Agent Update.}
The agent state update and response generation
($f_{\mathrm{agent}}, g_{\mathrm{agent}}$) incur a cost denoted
$O(A)$, which depends on the specific LLM or policy network. For a transformer LLM with context length $L_c$, complexity is typically $O(L_c^2 d)$.

\paragraph{Memory Write.}
The write operations to STM and LTM consist of:
\begin{itemize}
    \item Computing write candidates and gates: $O(d)$.
    \item Appending to STM (with truncation): $O(1)$ amortized.
    \item Appending to LTM index: $O(d)$ for vector insertion, plus the cost
    of index maintenance (often $O(\log N_L)$ per insertion for ANN indices).
\end{itemize}
Episodic memory updates occur once per episode instead of per step, and thus do not dominate per-step complexity.

\paragraph{Overall.}
For exact retrieval, the dominant term per step is
\[
O\big(E + A + (N_K + N_S + N_L)d\big),
\]
where typically $N_K \gg N_S, N_L$. With approximate nearest neighbor methods, the retrieval cost is reduced to sublinear in $N_K$ and $N_L$, making the agent update $O(A)$ and encoding $O(E)$ the main bottlenecks.

In distributed settings, Cylon and related data engineering tools parallelize the retrieval and indexing workload across nodes, effectively reducing $N_K$ and $N_L$ per node and amortizing the memory operations over multiple workers.




    
\end{comment}


==> tex/Dissertation/relatedwork.tex <==

\section{Related Works}
\label{sec:relatedWorks}

Modern deep learning and distributed computing research has increasingly focused on scalable frameworks and architectures for large-scale AI systems. The Ray framework improves heterogeneous workload management across clusters, enabling efficient distributed reinforcement learning \cite{moritz2018ray}. Similarly, Google’s Pathways architecture adopts a Multiple Program, Multiple Data (MPMD) design to support multimodal workloads while optimizing hardware utilization \cite{barham2022pathways}. Data processing frameworks remain central to large-scale AI pipelines. Apache Spark provides efficient in-memory processing for large datasets \cite{zaharia2016apache}, while Apache Flink enables real-time stream processing for applications such as anomaly detection \cite{carbone2015apache}. Dask further complements these systems by enabling parallel execution of complex analytical workloads \cite{rocklin2015dask}.

GPU-accelerated data processing has been advanced by cuDF, which reduces preprocessing latency and integrates seamlessly with deep learning frameworks such as TensorFlow and PyTorch \cite{sarker2022incremental}. Distributed preprocessing using Dask-cuDF has demonstrated significant speedups and near-linear scalability for LLM workloads \cite{daskcudf:online}. Additionally, frameworks like OneFlow improve large-scale transformer training through efficient memory and parallel computation \cite{yuan2021oneflow}. At the communication and orchestration level, ZeroMQ reduces latency in distributed systems \cite{zmq1:online}, while Parsl enables dynamic task scheduling for decentralized training workloads \cite{babuji2019parsl}.

Recent work on Retrieval-Augmented Generation (RAG) addresses limitations in handling long-context and complex queries. MemoRAG introduces a dual-system design to improve memory utilization \cite{qian2025memorag}, while RAG-Tuned-LLM enhances performance through RAG-style training \cite{wei2025tuning}. HippoRAG improves associative and factual memory via enhanced retrieval mechanisms \cite{gutierrez2025rag}, and Cue RAG introduces cue-based memory to retrieve deeper contextual knowledge \cite{fu2025cue}. Finally, these advancements highlight the importance of integrating distributed data processing, efficient communication, and adaptive retrieval mechanisms. Systems such as Cylon, Apache Arrow, and LlamaIndex contribute to this ecosystem, while AAFLOW extends these ideas by enabling more efficient, agent-driven execution for RAG pipelines.
